On Data-Driven Model Identification for Nonlinear Optimal Control

In this paper, we study the use of nonlinear model identification techniques for the optimal control of nonlinear systems, also known as model-based Reinforcement Learning. We show that the nonlinear model identification problem is equivalent to estimating the generalized moments of an underlying sampling distribution and is bound to suffer from ill-conditioning and variance when approximating a system to high order and over a large domain, requiring samples combinatorial-exponential in the order of the approximation and domain size: a ``Curse of Variance and Ill-Conditioning (COVIC)" that shows up even in very low dimensional problems, quite apart from the usual ``Curse of Dimensionality". We show that the iterative identification of ``local" linear time varying (LTV) models around the current estimate of the optimal trajectory, coupled with a suitable optimal control algorithm such as iterative LQR (ILQR), alleviates these issues and is sufficient to locally accurately solve the underlying optimal control problem.

==> Acknowledgements.tex <==
\section{Acknowledgements}
This work was partially supported by inputs and moral support by M.N.G. Mohamed, which helped the author overcome his crippling existential crisis.
Also, coffee helped.

==> Algorithm.tex <==
\section{The Reduced Order ILQR Algorithm}
\textcolor{red}{You should describe the main steps of ILQR and then how you modify the steps to obtain your RO-ILQR algorithm, currently your algorithm is indecipherable!}
The ILQR algorithm as it stands unfortunately faces the same issue of the Curse of Dimensionality when we scale the optimal control problems of PDEs to realistic resolutions. This is especially significant in the LTV system identification about a trajectory. 

\textcolor{red}{you should briefly describe ILQR here in words.} Let the PDE be discretized and modeled as an $N$-dimensional set of ODEs, with $p$ control inputs. The corresponding LTV system around an arbitrary trajectory is given by:

% Given a trajectory $\{x_t\}_{t=0}^T$ corresponding to control input $\{u_t\}_{t=0}^{T-1}$, we can use input-output perturbation and a Linear Least Squares method to estimate the LTV system given as

\begin{equation}
    \delta x_{t+1} = A_t \delta x_t + B_t \delta u_t
\end{equation}
where $A_t\in \mathbb{R}^{N\times N}$ and $B_t\in \mathbb{R}^{N\times p}$. To estimate the parameters $A_t$ and $B_t$, we can use input-output perturbation and a Linear Least Squares approach. Thus, we need at least $O(N+p)$ rollouts to identify the LTV system parameters.
\textcolor{red}{Explain how you would estimate these parameters using rollouts.}\\
When we scale up the PDE discretization, the increase in dimensionality leads to a quadratic increase in the number of parameters needed to be identified, thus requiring increasingly large number of samples to do so. Thus, the LTV system identification takes up an inordinate amount of time, which makes the ILQR approach intractable for PDEs. thus, in the following, we propose a POD based LTV identification technique that drastically reduces the computational burden of the LTV identification.

\textcolor{red}{The language and description in the following is too loose, you are writing a scientific paper! Please carefully describe the different steps below ``in the body of the paper", not in some algorithm!}

\subsection{Reduced Order LTV System}
\input{PerturbationModel.tex} 

\subsection{Compensation for basis change}
\textcolor{red}{What follows in IV B and C reads like gibberish, please describe carefully in terms of the iLQR algorithm steps.}
The reduced order basis used to project the dynamics and find the local LTV approximation can change significantly when changing the original trajectory, thus rendering the reduced order model invalid. For small perturbations to the trajectory, we can use the same set of basis for a decent approximation, but need to compensate for larger perturbations, such as the new trajectory after an iteration of the ILQR algorithm. 
In order to keep the model up-to-date with the new trajectory, we implement a repeated use of the snapshot-POD to compute the basis corresponding to that trajectory.
The new projection to the reduced order, LTV system identification and computations within the iterate thus make use of the shifted basis.

\subsection{Backward pass}
From the reduced order approximation of the initial trajectory, we can write the Bellman equation
\begin{equation*}
    J_t (\Phi \alpha_t)= \min_{u_t} \{c_t(\Phi \alpha_t, u_t)+J_{t+1} (\Phi \alpha_{t+1})
\end{equation*}
where $\alpha_{t+1}$ can be retrieved from the reduced order dynamics in Eq. 4. We can thus write the perturbed


% The backward-pass for the roILQR algorithm is summarized in Algorithm \ref{roILQR3}.

Thus, we summarize the roILQR algorithm as given in Algorithms \ref{roILQR1}, \ref{roILQR2} and \ref{roILQR3}.

\begin{algorithm}
  \caption{\strut Reduced-order ILQR with Shifting Basis}
  
  {\bf Initialization:} Set state $x = x_0$, initial guess $u^0_{0:T-1}$, line search parameter $\alpha = 1$, regularization $\mu = 10^{-6}$, iteration counter $k = 0$, convergence coefficient $\epsilon = 0.001$, line search threshold $\sigma_1=0.3$.\\
  
  Initial trajectory: $\{x_t^0\}_{t=0}^T=simulate\_forward\_step(x_0,u^0_{0:T-1})$\\
  Initialize the basis: $\Phi^{(0)} = snapshot\_pod(\{x_t^0\}_{t=0}^T)$\\
  \While {$cost_{k}/cost_{k-1} < 1 - \epsilon$}{
  \CommentSty{/* backward pass */}\\
  \{$k^{k}_{0:T-1}, K^{k}_{0:T-1}$\} $=$ backward\_pass()\\
  \CommentSty{/* forward pass */}\\
  Initialize $z=1$.\\
      \While{$z < \sigma_1$}{
            Reduce $\alpha$, \\
            $u^{k+1}_{0:T-1}$, $cost_k$, $\Delta cost(\alpha)$ $=$ forward\_pass($u^{k}_{0:T-1},\{k^{k}_{0:T-1}, K^k_{0:T-1}\}$),\\
            $z=(cost_k-cost_{k-1})/\Delta cost(\alpha),$\\
        }
        $k \leftarrow k + 1.$
      }{
      $\bar{u}_{0:T-1} \gets u^{k+1}_{0:T-1}$\\
  }
  
  
  
  \label{roILQR1}
\end{algorithm}

\begin{algorithm}
% \footnotesize
 \caption{\strut Forward Pass}
  {\bf Input:} Previous iteration nominal trajectory - $u^{k}_{0:T-1}$, iLQR gains - $\{k_{0:T-1}, K_{0:T-1}\}$.\\
  Start from $t = 0$, $cost = 0$, $\Delta cost(\alpha)=0$, $\bar{x}_0 = x_0$.\\
  \While {$t < T$}{
    \begin{equation*}
    \begin{split}
        u^{k+1}_{t} &= u_t^{k} + \alpha k_t + K_{t} ({x^{k+1}_t} - {x_t^{k}}),\\
        {x^{k+1}_{t+1}} &= simulate\_forward\_step(x^{k+1}_{t}, {u_t^{k+1}}),\\
        cost &= cost + incremental\_cost({x^{k+1}_{t}}, {u_t^{k+1}}),\\
        \end{split}
    \end{equation*}
    $t \leftarrow t + 1$. 
    }
  Basis Update: $\Phi^{(k+1)} = snapshot\_pod(\{x_t\}_{t=0}^T)$\\
  $cost = cost + terminal\_cost({x^{k+1}_T}),$\\ \vspace{2pt}
  $\Delta cost(\alpha) = -\alpha \sum_{t=0}^{T-1} k_t' Q_{u_t}-\frac{\alpha^2}{2}\sum_{t=0}^{T-1}k_t'Q_{u_tu_t}k_t.$\\
  {\bf return} $u^{k+1}_{0:T-1}$, $cost$, $\Delta cost(\alpha)$
  \label{roILQR2}
\end{algorithm}
%

\begin{algorithm} 
% \footnotesize
  \caption{\strut Backward Pass}
  \CommentSty{/* start from the terminal time */}\\
  $t \gets T - 1$.\ \\
  Compute $J_{\bf x_T}$ and $J_{\bf x_T x_T}$ using boundary conditions.\\
  \While {$t >= 0$}{
  \CommentSty{/* Estimate the Jacobians using LLS-CD as shown in Section \ref{sec4}-1): */}\\
  $\bar{A}_t, \bar{B}_t \gets LLS-CD({ \bar{\alpha}_t},{\bar{u}_t}).$\\
  \CommentSty{/* Obtain the partials of the Q function as follows: */}
    \begin{equation*}
    \begin{split}
    Q_{\alpha_t} &= c_{\alpha_t}  + \bar{A}^T J_{\alpha_{t+1}},\\
    Q_{u_t} &= c_{u_t} + \bar{B}_t^T J_{\alpha_{t+1}},\\
    Q_{\alpha_t \alpha_t} &= c_{\alpha_t \alpha_t} + \bar{A}_t^T J_{\alpha_{t+1} \alpha_{t+1}} \bar{A}_t, \\
    Q_{u_t \alpha_t} &= c_{u_t \alpha_t} + \bar{B}_t^T (J_{\alpha_{t+1} \alpha_{t+1}} + \mu I_{l \times l}) \bar{A}_t, \\
    Q_{u_t u_t} &= c_{u_t u_t} + \bar{B}_t^T (J_{\alpha_{t+1} \alpha_{t+1}}+ \mu I_{l \times l}) \bar{B}_t.\\
    \end{split}
\end{equation*}
  \eIf{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t \alpha_t}.
    \end{split}
    \end{equation*}
    Decrease~$\mu$.
    }
    {
    Increase $\mu$.\\
    Restart backward pass for current time-step.
    }
  \CommentSty{/* Obtain the partials of the value function $J_t$ as follows: */}
  \begin{equation*}
      \begin{split}
          J_{\alpha_t} &= Q_{\alpha_t} + K_{t}' Q_{u_t u_t} k_t + K_t' Q_{u_t} + Q_{u_t \alpha_t}' k_t,\\
          J_{\alpha_t \alpha_t} &= Q_{\alpha_t \alpha_t} + K_t' Q_{u_t u_t} K_t + K_t' Q_{u_t \alpha_t} + Q_{u_t \alpha_t}' K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  {\bf return} $\{k_{0:T-1}, K_{0:T-1}\}$.
  \label{roILQR3}
\end{algorithm}


==> Conclusions.tex <==
\section{CONCLUSIONS}
In this article, we have proposed an efficient approach for controlling nonlinear partial differential equations by employing model order reduction in tandem with a well known nonlinear optimal control algorithm ILQR. We have shown the viability and repeatability of the approach, and have compared it with a standard ILQR without model reduction to show that the proposed approach is highly efficient without sacrificing performance. In future work, we plan to apply the methodology to larger scale models, and also theoretically characterize the quality of the solution achieved here, and the sub-optimality thereof. Another future direction of work is the implications of the POD based reduced order LTV identification introduced here for nonlinear model reduction problems.

% In this article, we have provided an overview of the modeling of multi-phase micro-structures in accordance with the Allen-Cahn and Cahn-Hilliard equations. We have also compared learning/ data-based approaches to the control of such structures, outlining their relative merits and demerits. In future work, we shall further develop a hybrid model-data based method which can exploit a priori knowledge of the dynamics to significantly reduce computation time. We also plan to extend the methodology for higher-dimensional materials, leading up to an implementation on a realistic full-scale model.

==> DDPGAlgorithm.tex <==
\subsection{\textbf{DDPG Algorithm}}
\label{sec:ddpg}
Deep Deterministic Policy Gradient (DDPG) is a policy-gradient based off-policy reinforcement learning algorithm that operates in continuous state and action spaces. It relies on two function approximation networks one each for the actor and the critic. The critic network estimates the $Q(s, a)$ value given the state and the action taken, while the actor network engenders a policy given the current state. Neural networks are employed to represent the networks. 

The off-policy characteristic of the algorithm employs a separate behavioral policy by introducing additive noise to the policy output obtained from the actor network. The critic network minimizes loss based on the temporal-difference (TD) error and the actor network uses the deterministic policy gradient theorem to update its policy gradient as shown below:

Critic update by minimizing the loss: 
\begin{equation*}
    L = \frac{1}{N} \Sigma_{i}(y_i - Q(s_i, a_i| \theta^{Q}))^2
\end{equation*}

Actor policy gradient update:
\begin{equation*}
    \nabla_{\theta^{\mu}} \approx \frac{1}{N} \Sigma_i \nabla_a Q(s,a|\theta^{Q})|_{s=s_i,a=\mu(s_i)} \nabla_{\theta^{\mu}} \mu(s|\theta^{\mu})|_{s_i}
\end{equation*}

The actor and the critic networks consist of two hidden layers with the first layer containing 400 ('{\it relu}' activated) units followed by the second layer containing 300 ('{\it relu}' activated) units. The output layer of the actor network has the number of ('tanh' activated) units equal to that of the number of actions in the action space.  

Target networks one each for the actor and the critic are employed for a gradual update of network parameters, thereby reducing the oscillations and a better training stability. The target networks are updated at $\tau = 0.001$. Experience replay is another technique that improves the stability of training by training the network with a batch of randomized data samples from its experience. We have used a batch size of 32 for the inverted pendulum and the cart pole examples, whereas it is 64 for the rest. Finally, the networks are compiled using Adams' optimizer with a learning rate of 0.001. 

To account for state-space exploration, the behavioral policy consists of an off-policy term arising from a random process. We obtain discrete samples from the Ornstein-Uhlenbeck (OU) process to generate noise as followed in the original DDPG method. The OU process has mean-reverting property and produces temporally correlated noise samples as follows:
\begin{equation*}
    dx_t = \Theta (\mu - x_t)dt + \sigma dW
\end{equation*}
where $\Theta$ indicates how fast the process reverts to mean, $\mu$ is the equilibrium or the mean value and $\sigma$ corresponds to the degree of volatility of the process. $\Theta$ is set to 0.15, $\mu$ to 0 and $\sigma$ is annealed from 0.35 to 0.05 over the training process. 

==> FAQ <==
***********************************************************************
Question 1:
Could  you please send the information regarding importing 
encapsulated postscript (*.eps) files (figures)  
into your *.tex and *.sty (asme.tex or asme.sty) provided. 
What should be the command I should add to the file and in which file, 
in *.sty or *.tex. Usually I add \input epsf in my *.tex file. 
Please let me know this way of importing the figure is acceptable.

Answer:
You may use the 'epsfig' package to incorporate an encapsulated postscript
figure into your document.  To include the package in LaTeX2e, use
"\usepackage{epsfig}" in the preamble of your document.  Use
"\epsfig{file=file.eps}" to incorporate the eps file in the figure environment.  
You may use width and/or height arguments to change the size
of the original figure, e.g. "\epsfig{file=file.eps,width=3in}."

If you are using LaTeX 2.09, use "\input{psfig}" in the preamble and use
"\psfig{figure=file.eps}" to include the eps file.  The height and width
arguments are the same.

Note: the argument for \epsfig{} and \psfig{} starts with 
"file=" and "figure=", respectively.

***********************************************************************
Question 2:
I am current preparing a paper to be submitted in an ASME conference.
There is a problem we are not able to solve. The problem is the
display of lower case Greek bold face font. 
Normally, the command 
\mbox{\boldmath${  ....  }$\unboldmath}
will do it. However, using the ASME template, this command seem not
function. I wonder if you had come across this problem before and
would share you experience with us.

Answer:
In LaTeX2e, use the \mathbf{} command
to make a bold math character.  
If that doesn't work, you will have to use an ams-LaTeX package.  

***********************************************************************
Question 3: 
How can I get bold italics?

Answer:
try \newcommand{\bAC}{\mbox{$\mathbf{AC}$}}
You could also try \textbf{\emph AC}

***********************************************************************
Question 4: 

I've been using your LaTeX2e asme2e.cls package to prepare a paper
for an upcoming conference, but have been having some trouble with the
fonts.  I was wondering if I might be able to ask you for a bit of
advice.

It seems as if none of the headings, titles, etc, are showing
up bold as they are supposed to.  When I run LaTeX, I get the
following...

{co.eng.caltech.edu:7} latex paper.tex
This is TeX, Version 3.1415 (C version 6.1)
(paper.tex
LaTeX2e <1994/12/01> patch level 1
(asme2e.cls
Document Class: asme2e 1997/04/10 v1.0 Standard LaTeX document class
(/ccovol/tex3/tex/latex/base/ifthen.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/times.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/mathptm.sty)
(/ccovol/tex3/tex/latex/packages/psnfss/pifont.sty
No file Upzd.fd.

LaTeX Font Warning: Font shape `U/pzd/m/n ' undefined
(Font)              using `U/cmr/m/n' instead on input line 57.

No file Upsy.fd.

LaTeX Font Warning: Font shape `U/psy/m/n ' undefined
(Font)              using `U/cmr/m/n' instead on input line 58.




...and so on.

I noticed in the README2 file that there were some issues pertaining
to fonts.  Apparently I need to make sure that a new font package
(PSNFSS) is installed.  Does LaTeX's call to 

(/ccovol/tex3/tex/latex/packages/psnfss/times.sty)

imply that the sysadmins here have already done this?  In any case, I
tried to find the font packages at

http://tug2.cs.umb.edu/ctan/tex-archive/macros/latex/packages/psnfss/

but that address appears to have expired.  

If it is just a matter of installing these fonts, do you know of a new
address where I can get them?  And if it doesn't seem to be just a
problem of installing these fonts, do you have any ideas as to what
might be wrong?


Answer:
The problem is the  "pifont.sty" package uses the "Upzd.fd" and the "Upsy.fd"
font description files, which are missing in your installation of psnfss.  A
quick fix is to download the missing files from CTAN.  Point your browser to
http://www.ctan.org and click on the search link to search for the two files.
Download them to the same directory as your paper and rerun LaTeX2e.
You should ask your system administrators to install psnfss with the proper font
description files.



***********************************************************************
Question 5: 

How do you use .jgp and .png images as figures in LaTex when using PDF Texify?

Answer by Adam Pautsch at agpautsch@wisc.edu:
To include images, you must load the package "graphicx" in the preamble of 
the document. With the image file in the same folder as the .tex file, use 
the line "\includegraphics[keepaspectratio,width=3in]{filename.jgp}" to 
insert the image file. This may be included inside of a "figure" environment, 
which will allow for automatic captioning with the "\caption{}" command.

The images included in this manner will only appear when the "draft" option is
not used. When "draft" is used as an option, a box represnting an image with
the image's filename will appear in its place.

More information about handling images of different formats may be found at
     http://www.tex.ac.uk/cgi-bin/texfaq2html?label=dvipsgraphics
     http://www.tex.ac.uk/cgi-bin/texfaq2html?label=pdftexgraphics



==> ILQR.tex <==
\subsection{Iterative Linear Quadratic Regulator Details}

% The Iterative LQR algorithm implemented here is a variation of the classical Differential Dynamic Programming(DDP) algorithm, wherein we constrain ourselves to just the first derivative of the dynamics.
% Let $U_t=\{u_i\}_{i=t}^{T-1}$. The cost-to-go is, thus, defined as
% \begin{equation*}
%     J_t(x,U_t)=\sum_{i=t}^{T-1} c(x_t, u_t)+\phi(x_T)
% \end{equation*}

% The value function at time \textit{t} is the cost-to-go given the minimising control sequence,
% \begin{equation*}
%     V_t(x) \equiv \min_{U_t} J_t(x, U_t).
% \end{equation*}

% Setting $V_T(x)=\phi(x_T)$, we can apply the Dynamic Programming Principle, which reduces the minimization over a sequence of controls to a sequence of minimizations over a single
% control, proceeding backwards in time:
% \begin{align*}
%     V_t(x)=\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))], \\
%     Q_t(x)=arg\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))]
% \end{align*}
% We define the action-value function as a function of perturbations around the pair $(x_t, u_t)$:
% \begin{align*}
%     Q_t(\delta x_t, \delta u_t)=c(x_t+\delta x_t, u_t+\delta u_t)-c(x_t, u_t) +\\
%     V_{t+1}(f(x_t+\delta x_t, u_t+\delta u_t))-V_{t+1}(f(x_t, u_t))
% \end{align*}
% and expand to the second order
% \begin{align}
%     Q_t(\delta x_t, \delta u_t) \approx \frac{1}{2}\begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}^T \begin{bmatrix}
%     0 &Q_x^T &Q_u^T\\
%     Q_x &Q_{xx} &Q_{xu}\\
%     Q_u &Q_{ux} &Q_{uu}
%     \end{bmatrix} \begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}
% \label{eq:ilqg_2nd_order}
% \end{align}
% The expansion coefficients can be written as 
% \begin{align}
%     &Q_x = c_x+f_{x}^T V'_{x} \label{eq:ilqg1} \\
%     &Q_u = c_u+f_{u}^T V'_{u} \label{eq:ilqg2} \\
%     &Q_{xx} = c_{xx}+f_{x}^T V'_{xx}f_{x} + V'_x \cdot f_{xx}  \label{eq:ilqg3} \\
%     &Q_{ux} = c_{ux}+f_{u}^T V'_{xx}f_{x}  + V'_x \cdot f_{ux} \label{eq:ilqg4} \\
%     &Q_{uu} = c_{uu}+f_{u}^T V'_{xx}f_{u}  + V'_x \cdot f_{uu}\label{eq:ilqg5} 
% \end{align}
% where $V' \equiv V_{t+1}$. The final terms in equations \ref{eq:ilqg3}, \ref{eq:ilqg4} and  \ref{eq:ilqg5} are ignored in ILQR. 

% Minimizing equation \ref{eq:ilqg_2nd_order} w.r.t. $\delta u$ gives
% \begin{equation}
%     \delta u^* = arg \min_{\delta u} Q_t(\delta x,\delta u) = -Q_{uu}^{-1}(Q_u+Q_{ux}\delta x)
% \end{equation}
% This gives an open-loop term $k=-Q_{uu}^{-1}Q_u$, along with the feedback gain term $K=-Q_{uu}^{-1}Q_{ux}$. Substituting the policy in equation \ref{eq:ilqg_2nd_order}, we have a quadratic model of the value function:
% \begin{align*}
%     &\Delta V(t) = -\frac{1}{2} Q_u Q_{uu}^{-1}Q_u \\ %\label{eq:ilqg1} \\
%     &V_x(t) = Q_x-Q_u Q_{uu}^{-1}Q_{ux} \\%\label{eq:ilqg2} \\
%     &V_{xx}(t) = Q_xx-Q_{xu} Q_{uu}^{-1}Q_{ux}  %\label{eq:ilqg3}
% \end{align*}

% The backward pass recursively computes the local quadratic models of $V(t)$ and ${k(t), K(t)}$. When the backward pass is completed, a forward pass of the algorithm then computes a new trajectory:
% \begin{align*}
%     &\hat{x}(0)=x(0) \\
%     &\hat{u}_t = u_t+k(t)+K(t)(\hat{x}(t)=x(t))\\
%     &\hat{x}(t+1)=f(\hat{x}(t), \hat{u}_t)
% \end{align*}


We present details of the D2C-ILQR algorithm in the following. The pseudo-code is given in Algorithm \ref{model_free_DDP_OL}. The `forward pass' and `backward pass' algorithms are summarized in Algorithms \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively. Algorithm \ref{model_free_DDP_feedback} presents the DDP feedback algorithm used to calculate the optimal feedback gain. 
\begin{algorithm}[!ht]
\footnotesize
  \caption{\strut Open-loop trajectory optimization via model-free ILQR}
  {\bf Input:} Initial State - ${\bf x_0}$, System parameters - $\mathcal{P}$\;
  $m \gets 1$. ~~\CommentSty{/* Initialize the iteration number $m$ to 1.*/}\\
  $forward\_pass\_flag$ = true. \\
  \CommentSty{/* Run until the difference in costs between subsequent iterations is less an $\epsilon$ fraction of the former cost.*/}\\
  \While {$m==1$ {\textnormal{or}} $({\text cost}(\mathbb{T}_{nom}^{m})/{\text cost}(\mathbb{T}_{nom}^{m-1})) < 1 + \epsilon$}{
  \CommentSty{/*Each iteration has a backward pass followed by a forward pass.*/}\\
  \{$k^{m}_{0:N-1}, K^{m}_{0:N-1}$\}, $backward\_pass\_success\_flag$ $=$ Backward Pass($\mathbb{T}_{nom}^{m}$, $\mathcal{P}$).\\
  \If{backward\_pass\_success\_flag == true}{
      $\mathbb{T}_{nom}^{m+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{m}$,$\{k^{m}_{0:N-1}, K^m_{0:N-1}\}$, $\mathcal{P}$).\\
      \While{forward\_pass\_flag == false}{
            $\mathbb{T}_{nom}^{m+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{m}$,$\{k^{m}_{0:N-1}, K^m_{0:N-1}\}$, $\mathcal{P}$).\\
            Reduce $\alpha$ from $\mathcal{P}$.    
        }
      }
  \Else{
        Increase $\mu$ from $\mathcal{P}$.~~\CommentSty{/* Regularization step */}\\
    }
      $m \leftarrow m + 1$. \\
  $\mathbb{T}^{*}_{nom} \gets \mathbb{T}^{m+1}_{nom}$.\\
  }
  
  {\bf return $\mathbb{T}^{*}_{nom}$}\\
  \label{model_free_DDP_OL}
\end{algorithm}

\begin{algorithm}[!htp]
\footnotesize
 \caption{\strut Forward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$ and system and cost parameters - $\mathcal{P}$.\
%   \CommentSty{/* Unpack the previous nominal trajectory.*/}\\
  $\{{\bar{x}_t^{prev}, \bar{u}_t^{prev}}\} \gets \mathbb{T}_{nom}^{k}$.\\
%   \CommentSty{/* Initialize time to 0.*/}\\
  $t \gets 0$.\\
  \While {$t < N$}{
    %\CommentSty{/*$\alpha$ is the line-search parameter.*/} \\
    \CommentSty{/*Simulate one step forward ($\alpha$ is the line-search parameter.)*/}
    \begin{equation*}
    \begin{split}
        {\bar{u}_{t}} &= {\bar{u}_t^{prev}} + \alpha k_t + K_{t} ({\bar{x}_t} - {\bar{x}_t^{prev}}),\\
        {\bar{x}_{t+1}} &= simulate\_forward\_step({\bar{x}_t}, {\bar{u}_t}).
        \end{split}
    \end{equation*}
    $t \leftarrow t + 1$. 
    }
  $\mathbb{T}_{nom}^{k+1}$ $\gets$ $\{{\bf \bar{x}_{0:N}}, {\bf \bar{u}_{0:N-1}}\}.$\\
  \If{$\mathbb{T}_{nom}^{k+1}$ to $\mathbb{T}_{nom}^{k}$ \textnormal{is acceptable}}{
    {\bf return} $\mathbb{T}_{nom}^{k+1}$, true.
  }
  \Else{
    {\bf return} $\mathbb{T}_{nom}^{k}$, false.
  }
  \label{model_free_DDP_OL_FP}
\end{algorithm}
%
\begin{algorithm}[!htp]
\footnotesize
  \caption{\strut Backward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Backward pass starts from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\
  \CommentSty{/*Keep a copy of previous policy gains.*/}\\
  $k\_old \gets k_{0:N}$ {and}  $K\_old \gets K_{0:N}$.\\
  
  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $f_{x_t}, f_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } $\{ k\_old, K\_old\}$, false.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $k\_new = k_{0:N-1},$\\
  $K\_new = K_{0:N-1}.$\\
  {\bf return} $\{k\_new, K\_new\}$, true.
  \label{model_free_DDP_OL_BP}
\end{algorithm}

\begin{algorithm} [!htp]
\footnotesize
  \caption{\strut DDP Feedback}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Start from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\

  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $h_{x_t}, h_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the Hessians from simulator rollouts as shown above:*/}\\
  $h_{x_tx_t}, h_{u_tx_t}, h_{u_tu_t} \gets model\_free\_hessian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t} + J_{x_{t+1}}^{\prime}h_{x_tx_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t} + J_{x_{t+1}}^{\prime}h_{u_tx_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t} + J_{x_{t+1}}^{\prime}h_{u_tu_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } error.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $K = K_{0:N-1}.$\\
  {\bf return} $\{K\}$, true.
  \label{model_free_DDP_feedback}
\end{algorithm}

% \subsection*{Estimation of Jacobians: Linear Least Squares by Central Difference (LLS-CD)}
% \label{sys_id_solve_supplementary}

% \textit{Note: The following is a more detailed discussion of section 4.1.1 in the main paper.}
% % We make a preliminary analysis on the number of evaluations required in the above algorithm. If the horizon is `$h$' and the number of iterations required to converge are `$n$', the algorithm requires us to estimate each of the $f_{\bf x_t}$ and $f_{\bf u_t}$ `$nh$' times. 


% % \begin{equation*}
% % \begin{split}
% %     &f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) + \begin{bmatrix} f_{\bf x_t}  f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T  \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix} +
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %     &f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) - \begin{bmatrix} f_{\bf x_t} f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix}+
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %   \end{split}
% % \end{equation*}
% Using Taylor's expansions of `$h$' (for generality, $h$ is the non-linear model of Section 2) about the nominal trajectory $(\bar{x}_t,  \bar{u}_t)$ on both the positive and the negative sides, we obtain the following central difference equation:\\
% $
%     h(\bar{x}_t + \delta x_t, \bar{u}_t + \delta u_t) - h(\bar{x}_t - \delta x_t, \bar{u}_t - \delta  u_t) =~2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \\ \delta {u_t} \end{bmatrix} + O(\| \delta {x_t}\|^2 + \| \delta {u_t}\|^2).
% $
% Multiplying by $\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix}$ on both sides to the above equation:
% \begin{equation*}
%     \begin{split}
%     \begin{bmatrix}h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) -  h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix} 
%      \times \begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} 
%     % &= 2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} \begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix}+ O(\| \delta {\bf x_t}\|^4 + \| \delta {\bf u_t}\|^4)\\
%      =2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix} \nonumber \\~~~~~~~~~~~~
%      + O(\| \delta {x_t}\|^3 + \| \delta {u_t}\|^3)
%      \end{split}
% \end{equation*}
% Assuming that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible (which will later be proved to be true by some assumptions), let us perform inversions on either sides of the above equation as follows:
% % \begin{equation*}
% %     \begin{split}
% %     &\begin{bmatrix}f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) - f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t})\end{bmatrix} \times\\
% %     &\begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \delta {\bf x_t}^T & \delta {\bf x_t} \delta {\bf u_t}^T \\ \delta {\bf u_t} \delta {\bf x_t}^T  & \delta {\bf u_t} \delta {\bf u_t}^T \end{bmatrix}^{-1} = \\&2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} +
% %      O(\| \delta {\bf x_t}\|^2 + \| \delta {\bf u_t}\|^2)
% %      \end{split}
% % \end{equation*}
% % $\implies$ 
% \begin{equation}
%     \begin{split}
%     \begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} 
%     &=\frac{1}{2}\begin{bmatrix} h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) - h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix}  \times\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T~ \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T ~\delta {u_t} \delta {u_t}^T \end{bmatrix}^{-1}\\ &~~~~~~~~~~~~~~~~~~+ O(\| \delta {x_t}\| + \| \delta {u_t}\|)
%      \label{eq : model_free_DDP_jacobian_raw1}
%      \end{split}
% \end{equation}
% Equation \eqref{eq : model_free_DDP_jacobian_raw1} solves for Jacobians, $h_{x_t}$ and $h_{u_t}$, simultaneously. It is noted that the above formulation requires only 2 evaluations of $h(.)$, given the nominal state and control $\-$ (${\bar{x}_t},{\bar{u}_t}$). The remaining terms (also, the error in the evaluation) are of the order that is linear in $\delta {x_t}$ and $\delta {u_t}$. The following extends equation \eqref{eq : model_free_DDP_jacobian_raw1} to be used in practical implementations (sampling).\\
% We are free to choose the distribution of $\delta {x_t}$ and $\delta {u_t}$. We assume both are i.i.d. Gaussian distributed random variables with zero mean and a standard deviation of $\sigma$.~This ensures that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible. Let `$n_s$' be the number of samples for each of the random variables, $\delta {x_t}$ and $\delta {u_t}$. Denote the random samples as $\delta {X_t} = \begin{bmatrix} \delta {x_t^1}& \delta {x_t^2}& \ldots &\delta {x_t^{n_s}}\end{bmatrix}$, $\delta {U_t} = \begin{bmatrix} \delta {u_t^1} &\delta {u_t^2}& \ldots& \delta {u_t^{n_s}}\end{bmatrix}$ and $\delta Y_t = \begin{bmatrix} \delta X_t & \delta U_t \end{bmatrix}$. Then $\begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix}$ is given by the following (via standard least squares):
% \begin{equation}
%     \begin{split}
%     &\begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} = H \delta Y_t^T (\delta Y_t\delta Y_t^T)^{-1} \\
%     &H = \begin{bmatrix} h({\bar{x}_t} + \delta {x_t^1}, {\bar{u}_t} + \delta {u_t^1}) - h({ \bar{x}_t} - \delta {x_t^1}, {\bar{u}_t} - \delta {u_t^1})\\ h({\bar{x}_t} + \delta {x_t^2}, {\bar{u}_t} + \delta {u_t^2}) - h({\bar{x}_t} - \delta {x_t^2}, {\bar{u}_t} - \delta {u_t^2}) \\ \vdots  \\h({\bar{x}_t} + \delta {x_t^{n_s}}, {\bar{u}_t} + \delta {u_t^{n_s}}) - h({\bar{x}_t} - \delta {x_t^{n_s}}, {\bar{u}_t} - \delta {u_t^{n_s}})\end{bmatrix}
%      \label{eq : model_free_DDP_jacobian1}
%      \end{split}
% \end{equation}
% Let us consider the terms in the matrix $\delta Y_t \delta Y_t^T=\begin{bmatrix}  \delta {X_t} \delta {X_t}^T & \delta {X_t} \delta {U_t}^T \\ \delta {U_t} \delta {X_t}^T  & \delta {U_t} \delta {U_t}^T \end{bmatrix}$.~$\delta {X_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T$. Similarly, $\delta {U_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T$, $\delta {U_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T$ and $\delta {X_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T$. From the definition of sample variance, for a large enough $n_s$, we can write the above matrix as 
% \begin{equation*}
% \begin{split}
%     \delta Y_t \delta Y_t^T &= \begin{bmatrix} \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T \\ \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T
%     \end{bmatrix}\\ &\approx \begin{bmatrix} \sigma^2(n_s - 1) {\text I_{n_x}} & {\text 0_{n_x \times n_u}} \\ 0_{n_u \times n_x} & \sigma^2 (n_s - 1) {\text I_{n_u}}\end{bmatrix} \\
%     &= \sigma^2 (n_s - 1){\text I}_{(n_x+n_u) \times (n_x+n_u)}
% \end{split}
% \end{equation*}

% \textit{Sample Complexity.} 
% Given that we have high enough number of samples $n_s$, typically `$O(n_x + n_u)$', the above approximation holds good. The reason is as follows. Note that the above least squares procedure converges when the matrix $\delta Y_t \delta Y_t^T$ converges to the identity matrix. This is entirely equivalent to estimation of the covariance of the  random vector $[\delta x_t \ \delta u_t]$ where $\delta x_t$, and $\delta u_t$ are Gaussian i.i.d. samples. Thus, it follows that the number of samples is $O(n_x+n_u)$, given $n_x+n_u$ is large enough \cite{HDP-book}. \\
% Note that if one were to use an FD procedure, the number of samples would be $O(n_x(n_x+n_u)) >> O(n_x+n_u)$. In fact, this behaviour is clearly apparent in our empirical results where FD is more efficient for low dimensional examples, while the LLS-CD procedure rapidly becomes much more efficient as the size of the examples increases. This has very important ramifications since the overwhelming bulk of the computations in our D2C implementation is in the estimation of these system dynamics. 

% \subsection*{Guarantees for ILQR}
% %\textcolor{red}{Can you add the iLQR/ DDP insight here?}\\
% As has been mentioned previously, iLQR is much more efficient than the related DDP procedure \cite{ddp} which requires the availability of the second order dynamics terms. Albeit this is known empirically \cite{ilqg2}, it is not clear as to why iLQR should provide a solution of the same quality as DDP? \\
% The reasoning for this as follows. 
% The DDP procedure is simply a sequential quadratic programming (SQP) procedure for the trajectory optimization problem, where the dynamics are the constraints in the optimization problem. In SQP, the Lagrangian, i.e., the cost function augmented with the constraints using the Lagrange multipliers, $\mathcal{L}(x,\lambda) = c(x) + \lambda h(x)$, where $c(x)$ is the cost function and $h(x) =0$ are the constraints, is expanded to second order about the current solution. In the context of trajectory optimization, this amounts to expanding the cost function to second order which also results in second order expansion of the dynamics. The only difference between DDP and iLQR is that, in iLQR, the second order expansion of the dynamics is neglected in the optimization problem.
% This is similar to idea of neglecting second order terms in Gauss-Newton's method (identical to iLQR) as compared to Newton's method (identical to DDP).
% Moreover, the guarantees for SQP, i.e., convergence to a stationary point of the augmented cost function still holds for iLQR. Therefore, it follows that we can expect iLQR to converge to a stationary point of the optimal control problem.\\
% Next, note that due to the Method of Characteristics development in the previous section, if the dynamics are affine in control and the cost is quadratic in control, it follows that satisfying the necessary conditions for optimality, which iLQR is guaranteed to do under mild conditions, one is assured of the global minimum to the problem. Then, a perturbation expansion of the characteristic equations about this optimal is guaranteed to give us at least a local solution to the HJB equation.% due to Proposition~\ref{T-PFC}.
% %Since the inversion of an identity matrix is trivial and always exists, the above matrix is invertible in equation \eqref{eq : model_free_DDP_jacobian1}. Thus, one can calculate $f_{\bf x}$ and $f_{\bf u}$ this way during the backward pass. For the sake of convenience in the later sections, let us refer to this method as `Linear Least Squares by Central Difference (LLS-CD)'. 
% %The entire algorithm to determine the optimal nominal trajectory in a model-free fashion is summarized together in Algorithm \ref{model_free_DDP_OL}. The detailed forward and backward pass functions are shown in Algorithm \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively in the supplementary material.

\subsection*{DDP Feedback Gain Calculation}
Once the optimal nominal trajectory is obtained with ILQR, one DDP back pass is conducted to find the linear optimal feedback gain as shown in Algorithm \ref{model_free_DDP_feedback}. Then the linear feedback is wrapped around the nominal control sequence ($u_t = \bar{u}_t + K_t\delta x_t$),where $\delta x_t$ is the state deviation from the nominal state $\bar{x}_t$.

% \sr
% \begin{align}
% z_i &= \begin{bmatrix} \delta {x}^T & \delta {u}^T \end{bmatrix} \begin{bmatrix} h_{xx}^{(i)}  & h_{xu}^{(i)}  \\ h_{ux}^{(i)}  & h_{uu}^{(i)}  \end{bmatrix} \begin{bmatrix}  \delta {x} \\ \delta {u} \end{bmatrix} \nonumber \\  \nonumber
% &= \sum_{j=1}^{n_s} \sum_{k=1}^{n_s} \dfrac{\partial^2 h_i}{\partial x_j \partial x_k} \delta x_j \delta x_k + 2 \sum_{p=1}^{n_u} \sum_{q=1}^{n_s} \dfrac{\partial^2 h_i}{\partial u_p \partial x_q} \delta u_p \delta x_q + \sum_{d=1}^{n_u} \sum_{h=1}^{n_u} \dfrac{\partial^2 h_i}{\partial u_d \partial u_h} \delta u_d \delta u_h \\ \nonumber
% &= \underbrace{\begin{bmatrix} \delta {x_1}^2 & \delta {x_1} \delta {x_2} & \cdots & \delta {x_1} \delta {u_{n_u}} & \delta {x_2}^2 & \delta {x_2} \delta {x_3} & \cdots& \delta {u^2_{n_u}}\end{bmatrix}}_{\delta {XU}}  \underbrace{\begin{bmatrix} \dfrac{\partial^2 h_i}{\partial x_1^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial x_2} \\ \vdots \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial u_{n_u}} \\ \\ \dfrac{\partial^2 h_i}{\partial x_2^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_2 \partial x_3} \\ \vdots \\ \dfrac{\partial^2 h_i}{\partial {u^2_{n_u}}}\end{bmatrix}}_{H_i},\\
% \end{align}
% % \begin{bmatrix} \delta {x_1} & \delta {x_2} & \cdots & \delta {x_{n_s}} & \delta {u_1} & \delta {u_2} & \cdots & \delta {u_{n_u}} \end{bmatrix} 

% where $h_{xx}^{(i)} = \left.\dfrac{\partial^2 h_i}{\partial x^2}\right|_{x=t}$, $z_i$ is the $i^{th}$ element of vector $z_t$ and $h_i$ is the $i^{th}$ element of the dynamics vector $h(x_t, u_t)$. Multiplying on both sides by $\delta XU^T$ and apply standard Least Square method:
% $H_i = (\delta XU^T \delta XU)^{-1} \delta XU^T Z_i$. Then repeat for $i=1,2,...,n_s$ to get the estimation for the Hessian tensor.

==> Introduction_revised.tex <==
\section{Introduction}

% The modeling and control of infinite-dimensional partial differential equations has long been a topic of avid interest, extending into various different fields ranging from fluid flows \cite{lellouche}, protein folding and enzyme kinematics \cite{proteinfold}, to microstructure dynamics \cite{Boe2002}\cite{Rui2011}. Such problems are usually solved by employing numerical methods, discretizing the state space through finite-element methods and controlling the resulting very high-dimensional system of differential equations. The need for dimensionality reduction in such systems paved the way for Model Order Reduction techniques, accomplished in a data-driven manner, using techniques such as DMD \cite{dmd1}\cite{dmd2}, Neural Networks \cite{nn1}\cite{nn2}, nonlinear auto-regressive algorithms\cite{nara1}, and sparse regression\cite{sparse1}. Perhaps the most widely used approach is the so-called Proper Orthogonal Decomposition (POD) Method of Snapshots that finds a reduced basis for the approximation of the nonlinear PDE using snapshots from a simulation of the same\cite{sirovich1987turbulence}.

% \textcolor{red}{the original POD paper is not by Lall, its from Fluids, by Sirovich, please reference that paper.} }
% \textcolor{blue}{%Despite a lot of progress in the field, the control of nonlinear systems still remains a challenging problem. Methods for nonlinear control design, such as sliding mode control \cite{smcreview}\cite{nonlinearsmc}, backstepping and Lyapunov function analysis \cite{krstic1995nonlinear}\cite{vaidyanathan2020backstepping} have been developed and have been shown to work with a wide range of low-dimensional applications.}
In our previous work \cite{wang2021search}\cite{yu2019decoupled}, we proposed a data-based algorithm for optimal nonlinear control, which identifies successive linear time-varying (LTV) models combined with the so-called Iterative Linear Quadratic Regulator (ILQR) approach to yield a globally optimum local feedback law. The ILQR algorithm \cite{li2004iterative} is a sequential quadratic programming (SQP) approach, typically used to solve nonlinear programming problems, for the solution of optimal control problems, and under relatively mild conditions can be shown to converge to the global minimum of the optimal control problem \cite{wang2021search}. The ILQR is a versatile approach and has been successfully applied to a wide range of relatively low-dimensional robotic applications \cite{ilqr2}\cite{ilqr3}. %with several extensions to the algorithm, such as the iterative LQG \cite{todorov2005generalized} further diversifying the applications of the original algorithm. 
%The complexity of solving nonlinear control problems increases exponentially when tacked on with the Curse-of-Dimensionality, resulting from solving for very high-dimensional problems. 
Unfortunately, none of these extensions address the intractability of the ILQR algorithm when dealing with high-dimensional systems, in particular PDEs that require the identification of very high dimensional LTV models and leads to intractability of the critical backward pass Ricatti recursion in the algorithm. Hence, the optimal control of nonlinear PDEs still remains a major challenge.

\begin{figure}
    %\centering
    % \includegraphics[width=0.8\linewidth]{images/temporal_disc.png}
\begin{multicols}{4}
   
      \subfloat[Initial State]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj11.png}}
      \subfloat[Int. I]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj12.png}}
      \subfloat[Int. II]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj13.png}}
      \subfloat[Final State]{\includegraphics[width=\linewidth]{images/roilqr plots/Trajm14.png}}
      
      
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}
\begin{multicols}{4}
   
       
      \subfloat[1st mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis11.png}}
      \subfloat[2nd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis12.png}}
      \subfloat[3rd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis13.png}}
      \subfloat[4th mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis14.png}}
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}

\begin{multicols}{4}
   
      \subfloat[Initial State]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj201.png}}
      \subfloat[Int. I]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj202.png}}
      \subfloat[Int.  II]{\includegraphics[width=\linewidth]{images/roilqr plots/Traj203.png}}
      \subfloat[Final State]{\includegraphics[width=\linewidth]{images/roilqr plots/Trajm204.png}}
      
      
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}

\begin{multicols}{4}
   
       
      \subfloat[1st mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis201.png}}
      \subfloat[2nd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis202.png}}
      \subfloat[3rd mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis203.png}}
      \subfloat[4th mode]{\includegraphics[width=\linewidth]{images/roilqr plots/Basis204.png}}
      %\subfloat[Gradient-descent based D2C Convergence]{\includegraphics[width=1\linewidth]{images/episodic_cost_OL_training.png}}
      
\end{multicols}


    %\caption{Comparing control cost at different time-discretizations}
    \caption{\small The initial trajectory (a)-(d) differs significantly from the final trajectory optimized by ILQR (i)-(l). Thus, the set of basis eigenfunctions for the initial trajectory (e)-(h) will only be valid locally, and differ significantly from the reduced order subspace that the optimal trajectory lies on (m)-(p). Hence, it is key to update the reduced-order basis with each successive iteration of the algorithm.}
    \label{fig:up_top}

\end{figure}


The field of PDE control has a rich history, for instance, see Kunisch \cite{KunischOCPDE},%\cite{KunischSLPDE},
Volkwein \cite{volkweinPhaseField},%\cite{VolkweinParabolicADR},
%Krstic \cite{smyshlyaev2010adaptive}, Alla \cite{allaSLPDE} 
and Falcone \cite{allafalconeadaptive}. %This foundational work was further built upon for application to nonlinear PDE control \cite{Breiten}\cite{bennerOCPDE}\cite{VolkweinFeedbackController}\cite{volkweinNonlinearRDE}\cite{krstic2008backstepping}. 
Recent work from Kramer et al \cite{Kramer-ILQR} have suggested using a linear time invariant (LTI) model reduction technique called Balanced Truncation \cite{tacBT} %\cite{BTLQG}
 to obtain a reduced basis on which to project the nonlinear PDEs to obtain a reduced order nonlinear model, the optimal control for which is then accomplished using the ILQR algorithm.  However, in general, the reduced basis modes can be quite different around the optimal trajectory when compared to an initial trajectory, and an approximation using the latter’s reduced basis can lead to unacceptable performance \cite{ravindran2002}\cite{kunisch2008}. %(also see Fig. 1). 
 Therefore, the reduced basis needs to be adaptively changed as the optimization proceeds \cite{kunisch2008}\cite{pod_volkwein}. Moreover, for nonlinear PDEs, the model reduction still results in a lower order nonlinear model, whose optimal control is itself challenging, and in general, intractable. %Further, it is not clear how one improves on the reduced order model to converge to the optimal trajectory. 
\textit{In this regard, the simple yet fundamental observation we make is that since the Proper Orthogonal Decomposition (POD) basis is local, an LTV model suffices to approximate the local behavior of the nonlinear PDE rather than a reduced nonlinear model.} %This enables us to use a reduced order version of the ILQR approach where we recursively change the reduced basis for successive trajectories using the method of snapshots and obtain reduced order LTV systems around the current estimate. This allows to recursively use reduced order LTV control techniques to solve for the optimal nonlinear control in a highly efficient fashion.} }\\

Thus, in this paper, we introduce a reduced order Iterative Linear Quadratic Regulator (RO-ILQR) approach for the optimal control of nonlinear PDEs. The ILQR approach iteratively linearizes the dynamics and quadratizes the cost function around the current estimate of the optimal trajectory, solves a time varying LQR problem to find an improved control sequence, and repeats the process till convergence. In this paper, we use the POD Method of snapshots \cite{sirovich1987turbulence} to find a reduced order LTV approximation of the PDE around the current trajectory, solve a reduced order LQR problem to find an improved trajectory along with an updated POD basis, and iterate till convergence, thereby drastically reducing the computational burden of the ILQR approach when applied to PDEs. The proposed approach is tested on the viscous Burger's equation and on two phase field models for reaction-diffusion equations describing microstructure evolution in multi-phase materials and is shown to converge to the global optimum that would result without the model reduction.
%\noindent The contributions of the paper are as follows:
%\begin{itemize}
    % \item We show how to model the dynamics of a multi-phase micro-structure and unveil its underlying structure.
 %   \item We propose a reduced order ILQR (RO-ILQR) algorithm for the control of systems that are governed by complex, nonlinear PDEs, using the POD method of snapshots to find local reduced order LTV approximations of the nonlinear PDE around a current trajectory.
    
  %  \item We compare the proposed RO-ILQR approach to the full-order ILQR algorithm, and show that the reduced order approach significantly reduces the computational burden, albeit with a small loss in optimal performance owing to the model reduction, when operating on high-dimensional PDEs.  
   
%\end{itemize}



%\section{Related Work}
The rest of the paper is organized as follows: In Section \ref{sec2}, we introduce the PDE nonlinear optimal control problem. We discuss the issues related to control of high-dimensional PDEs, and suggest ways to navigate around them in Section \ref{sec3}. In Section \ref{sec4}, we briefly introduce the iLQR algorithm, followed by the proposed approach. Section \ref{sec5}
illustrates the application of the proposed approach through custom-defined test problems of varying dimensions, along with repeatability, followed by the benchmarking of the approach with the standard ILQR.

\vspace{-0.15cm}

==> Motivation.tex <==
% \section{Motivation}




% \begin{figure}[!htpb]
% \vspace{-0.5cm}
% % \begin{multicols}{2}
%     %\hspace{1.4cm} 
%       \subfloat[Initial Condition 1]{\includegraphics[width=\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_10degsingletraj1.png}}    
%     %   \subfloat[Goal state-I]{\includegraphics[width=\linewidth]{images/Final_state.PNG}} 
%     \\
%       \subfloat[Initial Condition 2]{\includegraphics[width=1.1\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_10degsingletraj6.png}}
      
% % \end{multicols}

% \caption{{MLP model trained and tested for a smaller trajectory neighbourhood.}}
% \vspace{-0.4cm}
% \label{fig:MLP@10}
% \end{figure}

When we increase the portion of the state-space captured in the dynamics, we observe that the predictions track well for the first few time-steps, but differs significantly with the horizon. Fig.~\ref{fig:MLP@90} shows this behavior when training on initial conditions with $\theta_0\in [-180^\circ, 180^\circ]$.


% \begin{figure}[!htpb]
% \vspace{-0.5cm}
% % \begin{multicols}{2}
%     %\hspace{1.4cm} 
%       \subfloat[Initial Condition 1]{\includegraphics[width=\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_180degsingletraj4.png}}    
%     %   \subfloat[Goal state-I]{\includegraphics[width=\linewidth]{images/Final_state.PNG}} 
%     \\
%       \subfloat[Initial Condition 2]{\includegraphics[width=1.1\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_180degsingletraj5.png}}
      
% % \end{multicols}

% \caption{{MLP model trained and tested for a larger trajectory neighbourhood.}}
% \vspace{-0.4cm}
% \label{fig:MLP@90}
% \end{figure}

As a sanity check, we considered a linearized model of the pendulum, and trained the MLP model on that system. We observe the trajectory being perfectly tracked in that case, as observed in Fig.~\ref{}.

==> Reviews_ACC.tex <==
Reviewer 1:

One remaining question could be a comparison of the
nonlinear optimal control using ILQR, to verify if the
model can still be controlled by ILQR with the sampling
error in the modeling data.

Reviewer 2 of ACC 2024 submission 1076

Comments to the author
======================

General Review
--------------
This paper reviews the use of nonlinear system
identification techniques in representing dynamic models in
optimal (model-based) control strategies. The paper
attempts to illustrate the deficiencies of nonlinear
data-driven models and then argues for linear time-varying
(LTV) models instead of nonlinear data-driven models. The
paper gives results on several case simulation-based case
studies.

In general, this paper appears to make a
comparison/argument between two categories of modelling
types. I failed to see clear reasoning behind comparing a
static dynamical model (i.e., a neural network and/or model
based on SINDy method) to a time-varying model, and
therefore, am unclear on the contributions of this work.

In general, this paper should try to reformulate the
message of the work restructure the writing with respect to
their unique contributions.


Detailed Review
---------------
Abstract
 - I think that the abstract is missing a sentence or two
on the background/motivation of the work.
 - It is unclear whether the author's statement on
"show[ing] that the nonlinear system identification problem
is equivalent to estimating the generalized moments ..." is
a novel contribution. If it is, then it should be clearly
stated; if not, then the author's need not spend half of
the paper to discuss this particular point.
 - The authors use the terms "necessary as well as
sufficient," which implies that a theorem is being proposed
in this work. In the abstract, it would be good to say that
a new theorem is proposed, if that is a novel contribution.
 - The authors could add a statement saying that they have
demonstrated their contributions using closed-loop
simulations of benchmark dynamic systems (such as CartPole,
Pendulum, Fish, etc.).

Introduction
 - I think there is some redundancy when the authors
mention that in this work they will be using SINDy and
neural networks as the nonlinear system identification
techniques (mentioned in first paragraph and second to last
paragraph). The authors could consolidate their discussion
in the introduction by first discussing the main
motivation(s) and some background behind the contributions
of the paper (i.e., what is nonlienar system
identification, why nonlinear dynamic models are
useful/necessary, how are they used, what advantages do
they have, why are they useful in control). Then, they can
reference the choices that they made in the main body of
the paper. Several of these are already addressed in the
existing submission, but it can be cleaned up and
reorganized to be more clear. Additionally, I think there
is a disconnect between the model identification aspect of
this work with the optimal control motivation. There should
be some discussion of how optimal control can benefit from
different types of dynamic models.

Section II: Preliminaries
 - The authors describe nonlinear system identification as
a key component of this work. If this work depends on that,
then it would be useful to provide a brief discussion on
that and where its deficiencies lie. I think this is
somewhat addressed in subsection B of this section, but it
is unclear where the strengths and weaknesses are, so it is
difficult to discern the problem that the authors are
addressing.
 - I would recommend defining the optimal control problem
with the appropriate constraints rather than stating in the
following text
 - It is unclear if the ILQR discussion is necessary in
this section. Alternatively, the discussion may be better
summarized in an Algorithm context.
 - "we iterate the process by repeating steps (1) to (4)"
do you mean (3)?
 - The authors may consider using \langle and \rangle for
the left and right angle brackets to make the notation
clearer.
 - Again, the description of the approximation problem may
be better summarized in an Algorithm context.


Section III: Data Driven Solutions
 - The title of this section is unclear to me. What is
"solutions" used in reference to? Is there a method
proposal(s) or alternative strategy(ies) proposed here?
 - The authors present this section with a lot of inline
math, which makes the text difficult to read. It would be
good if the authors could organize the ideas presented here
such that the math is not all inline with the text.
 - I would recommend making several functions (e.g., Prob,
Var, exp, Span) non-italic
 - The statement immediately following (5) is difficult to
read and is unclear where the subscripts came from. Is
\underline{\Psi} (no subscript) a set of
\underline{\Psi}_{ik} (with subscript)?
 - In Proposition 1, the sentence "Then, the solution of
the data-based ..." does not read as a complete sentence.
 - till --> until
 - It is unclear what the contribution of this section is.
My understanding is that there is distributional shift when
trying to control a system that has no analytical solution
(a well-known idea especially as the control agent explores
new regions of the state space). Hence, the authors argue
for the use of time-varying models. It is unclear why there
is significant focus on nonlinear static models and why the
authors choose to address the problem with time-varying
linear models.

Section IV: Empirical Results
 - In general, I think that this section could be improved
if the authors articulated the purpose of the figures and
then provided discussion as to what the key takeaways from
the figures are. Some of the former is there, but the
latter is missing. (e.g., what are the takeaways from Fig.
2? Why is there a difference? Does the LTV model perform
significantly better? In Fig. 3, what happened to the LTV
performance in (c) and (d)?)
 - In general, some of the text in the figures (namely the
axes labels, legend labels, title) have very small text and
are difficult to read, while the captions do not provide
explanation as to what the titles of the figures mean.
 - The poor performance of the MLP in Fig. 4 seems to
strongly support the arguments that the authors are trying
to make, but there is no comparison to the LTV model. Does
LTV work in this case?
 - The discussion on model convergence could be improved.
First, it is unclear what the authors claim that the
nonlinear models should "converge" to the same parameters
when trained on different datasets from the same
distribution is true. Second, what is the consequence of
this so-called convergence? Is there proof that the LTV
models would have a comparable quality? i.e., what
guarantees are there that the nonlinear models are bad in
this sense but the LTV models are good?
 - It would also be helpful if the authors give a short
justification for the levels of perturbations that they
evaluated. Why 30%? Why 10%? Why 100%? The choices seem
somewhat arbitrary.
 - With repsect to the optimal control results, the authors
should provide some perspective as to why the nonlinear
models do not work/converge.

Conclusions
 - Once the contributions and message of the work has been
clarified, then the conclusion should be modified
accordingly.
 - The authors use "suffice and necessary" when no theorem
has been given. Further, the authors only present one case
(CartPole) that supports that statement regarding the
optimal control problem. It would be more compelling if the
authors were able to demonstrate this on multiple cases as
they had originally alluded to at the beginning of Section
IV.

Reviewer 4 of ACC 2024 submission 1076

Comments to the author
======================

The authors have tried to use system identification tools
to solve iterative optimal control problem. However, there
is no analytical result (Theorems with proofs) in the
paper. This looks like an out of scope paper to me. 


Reviewer 12 of ACC 2024 submission 1076

Comments to the author
======================

The paper shows that data-driven nonlinear system
identification techniques such as SINDY and DNN need
samples combinatorial-exponential in the order of the
approximation and suffer from ill-conditioning of the Gram
matrix. The paper then empirically compares the prediction
error of SINDY, DNN, and LTV (derived from the authors'
ILQR approach) models given an optimal control input
sequence. While the mathematical derivation of the sample
complexity for nonlinear system id techniques appears to be
novel, some of the empirical evidence against these
techniques and comparison study done in the rest of the
paper does not seem to meaningfully support the superiority
of the ILTV approach, as the author claim.

1. SINDY's novelty is in the fact that it chooses a sparse
number of basis functions to arrive at the optimal
solution, stemming from the intuition that most dynamical
systems can be described with a small number of nonlinear
terms. The original paper
[https://doi.org/10.1073/pnas.1517384113] notes that a
simple linear combination of nonlinear basis functions and
its least-squares solution is prove to overfitting, and
introduces the concept of sparse identification to
drastically improve model accuracy with limited data.
Therefore, the derivations in II.B, which assumes a
least-square solution does not apply to SINDY.

2. Similarly, while MLPs are widely used for its
simplicity, it is already well understood in the community
that it does not perform well in limited data, and does not
generalize well to samples that are not in the training
set. Many algorithms have been proposed to tackle the
generalization problem (e.g. Lipschitz neural networks
[https://doi.org/10.48550/arXiv.1811.05381], also some
results exist for simultaneous system identification and
optimal control using neural networks (for e.g. Input
convex neural networks [https://arxiv.org/abs/1805.11835]).

3. Model convergence. All nonlinear function approximation
techniques arrive at different model parameters when given
a different finite set of data, even if it is sampled from
the same distribution. None of the methods (SINDY and MLP)
claim that models should converge to the same parameters
with different finite datasets. The convergence guarantees
of these techniques (if it exists) are, at best, asymptotic
in the number of points in the dataset.

4. Given that the black box model is already provided, and
that the training is done off-line prior to control
implementation, the requirement of a large sample does not
seem to be a major drawback, especially if one can
ultimately reach a highly accurate parametric nonlinear
model and solve for a nonlinear optimal control law that
can be used in a wider range of states than the ILQR
approach. Also, the surrogate model could be used to find
an infinite-time (or time-invariant) optimal controller,
while the ILQR cannot, due to the nature of the
forward-backward pass. 

5. The comparison in Fig. 11 seems intuitive, and does not
support the superiority of the ILQR approach. What is the
controller used in Fig. 11? If it is the ILQR approach,
naturally, the solution will diverge from the true optimal
trajectory as the model error increases. Why would one use
an imperfect surrogate model for ILQR if a more accurate
black-box model is already available? 

I think a fair comparison would be between the ILQR
approach and an optimal control strategy using the
surrogate models, which should employ nonlinear optimal
control methods that can be derived from a parametric
model, such as the Galerkin approach
[https://doi.org/10.1080/002071798221542]. A comparison of
the control cost should be given, as the black-box model
moves away from the true system.

6. Models (black-box or not) are always inaccurate, and
controllers need to be robust against the model error.
Judging from Fig. 11, and assuming that the ILQR was used
to find the control law for the surrogate models, the
result suggests that the ILQR approach is not robust
against model errors. Can the authors comment about the
robustness property of the ILQR approach in comparison to a
true nonlinear optimal (closed-loop) controller? 

==> Simulations.tex <==
\section{Empirical Results}\label{sec5}

In this section, we develop the experiments to generate our data-based nonlinear models in an optimal control perspective. Starting with our model descriptions, we train our benchmark algorithms on the MUJOCO-based simulator systems to compare performance. Then, we provide empirical justifications for the theory developed above.
%Starting from very simple, zero-control experiments, we build towards the control perturbation tests, and observe the performance of the selected algorithms on these experiments. 

% \subsection{Structure and Task}
% We simulated the dynamics in Python, through calling an explicit, second-order solver subroutine in FORTRAN. The system and its tasks are defined as follows: 
\subsection{Model Verification: MLP}
\subsubsection{Pendulum}
In general, data-based system identification techniques proceed to compute the dynamics the same way: Generate a set of trajectories through sampling the black box, and then project these onto a set of nonlinear basis functions to get the corresponding coefficients. The computation of these coefficients is carried out through techniques like gradient descent, linear least squares, etc. For a set of trajectories lying in a small neighborhood, these techniques are able to capture and predict the general dynamics extremely well. Unfortunately, the quality of the model degrades as we scale the neighborhood of these sample trajectories to capture a larger portion of the state-space, and the predictions tend to deviate very quickly.

This can be experimentally determined through the use of the simple pendulum problem, with no controls. For the prior case, the initial condition of the pendulum was randomly drawn from the linear regime, i.e. from a set $\theta_0\in [-10^\circ, 10^\circ]$. The pendulum is, thus, released from rest and tracked for 100 time-steps. A set of 1000 such trajectories is generated, with a 9:1 split for testing and training, and an MLP model is trained on this data. From Fig.~\ref{fig:MLP@10}, we observe that the dynamics match well even for a longer horizon.
\begin{figure}[!htpb]
% \vspace{-0.5cm}
% \begin{multicols}{2}
    %\hspace{1.4cm} 
      \subfloat[Initial Condition 1]{\includegraphics[width=\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_10degsingletraj1.png}}    
    %   \subfloat[Goal state-I]{\includegraphics[width=\linewidth]{images/Final_state.PNG}} 
    \\
      \subfloat[Initial Condition 2]{\includegraphics[width=1\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_10degsingletraj6.png}}
      
% \end{multicols}

\caption{{MLP model trained and tested for a smaller trajectory neighborhood.}}
\vspace{-0.4cm}
\label{fig:MLP@10}
\end{figure}

When we increase the portion of the state-space captured in the dynamics, we observe that the predictions track well for the first few time-steps, but differ significantly with the horizon. Fig.~\ref{fig:MLP@90} shows this behavior when training on initial conditions with $\theta_0\in [-180^\circ, 180^\circ]$.


\begin{figure}[!htpb]
\vspace{-0.5cm}
% \begin{multicols}{2}
    %\hspace{1.4cm} 
      \subfloat[Initial Condition 1]{\includegraphics[width=\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_180degsingletraj4.png}}    
    %   \subfloat[Goal state-I]{\includegraphics[width=\linewidth]{images/Final_state.PNG}} 
    \\
      \subfloat[Initial Condition 2]{\includegraphics[width=1\linewidth]{images/NN_Pendulum/Theta_indeg_icud2_180degsingletraj5.png}}
      
% \end{multicols}

\caption{{MLP model trained and tested for a larger trajectory neighborhood.}}
\vspace{-0.4cm}
\label{fig:MLP@90}
\end{figure}

\subsubsection{Cartpole}
We ran similar perturbation experiments for the MUJOCO cartpole system, jittered about the equilibrium point. To verify whether the MLP model works, we test our results on two fronts:
\\
Case I: With zero control-inputs (no force on the cart) and different initial conditions, the MLP model should be able to capture just the pendulum dynamics. This is successfully observed in Fig.~\ref{fig:MLP@120}, where we perturb the pole initially by angles sampled from $\theta_0\in [-120^\circ,120^\circ]$. We observe the trends to be similar to how the MLP model behaved in the pendulum system task.

\begin{figure}[!htpb]
\begin{multicols}{2}
    %\hspace{1.4cm} 
      \subfloat[Initial Condition 1]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/zero_ctrl/Theta_indeg_icud2_120degsingletraj1.png}}    
      \subfloat[Initial Condition 2]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/zero_ctrl/Theta_indeg_icud2_120degsingletraj2.png}}
\end{multicols}
\begin{multicols}{2}
    
      \subfloat[Initial Condition 3]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/zero_ctrl/Theta_indeg_icud2_120degsingletraj3.png}}    
      \subfloat[Initial Condition 4]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/zero_ctrl/Theta_indeg_icud2_120degsingletraj4.png}}
      
\end{multicols}

\caption{{MLP model trained and tested for zero controls on the cartpole system.}}
\label{fig:MLP@120}
\end{figure}

Case II: With small perturbations around the equilibrium, the MLP model should be able to capture the full-state dynamics. The cart is perturbed by $F \sim 0.1*rand()$, with initial conditions for the pendulum drawn from $\theta_0\in [-120^\circ,120^\circ]$. We observe the MLP model does not track the cart position and velocities well (Fig.~\ref{fig:MLP@Cartpole_jitter}).

\begin{figure}[!htpb]

\begin{multicols}{2}
    %\hspace{1.4cm} 
      \subfloat[Cart position]{\includegraphics[width=1.1\linewidth]{images/NN_Cartpole/small_perturbations/X_icud2_120degsingletraj_1.png}}    
      \subfloat[Pendulum position]{\includegraphics[width=1.1\linewidth]{images/NN_Cartpole/small_perturbations/Theta_indeg_icud2_120degsingletraj1.png}}
\end{multicols}
\begin{multicols}{2}
      \subfloat[Cart Velocity]{\includegraphics[width=1.1\linewidth]{images/NN_Cartpole/small_perturbations/dX_icud2_120degsingletraj_1.png}}
      \subfloat[Pendulum angular velocity]{\includegraphics[width=1.1\linewidth]{images/NN_Cartpole/small_perturbations/dTheta_indeg_icud2_120degsingletraj1.png}}
      
\end{multicols}

\caption{{MLP model trained and tested for small perturbations around the equilibrium on the cartpole system.}}
\label{fig:MLP@Cartpole_jitter}
\end{figure}

\subsection{Perturbation Experiments:}

\subsubsection{Benchmarking for the Pendulum system}
Using our optimal control algorithm, we generate the optimal trajectory and control for the modified pendulum swingup task: Starting from the downward position of the pendulum ($\theta_0=180^\circ$), the pendulum needs to swing-up and come to rest at $\theta_T = 60^\circ$ within 30 time-steps. We generate the training data by increasingly perturbing about the optimal trajectory, and sampling 2000 trajectories (60000 data-points) from the neighborhoods obtained. The sampled trajectories are then split in a 9:1 ratio for the testing and training set respectively. We train both the MLP model and SINDy on these data-points and generate the predictions to compare their performance. To benchmark these 'global' nonlinear models against a 'local' model, we compare them with a classic linear time-varying model generated from input-output perturbations and a least-squares fit.

\begin{figure*}[!htpb]
\vspace{-0.5cm}
\begin{multicols}{3}
    %\hspace{1.4cm} 
      \subfloat[Swingup with $10\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/theta_10pc1.png}}    
      \subfloat[Swingup with $20\%$ perturbation]{\includegraphics[width=1\linewidth]{images/NN_Pendulum/LTV/theta_20pc1.png}}
      \subfloat[Swingup with $30\%$ perturbation]{\includegraphics[width=1\linewidth]{images/NN_Pendulum/LTV/theta_30pc1.png}}
      \\
      \subfloat[Phase-phase plot for $10\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/Phase-Phase/Phase_phase_10.png}}
      \subfloat[Phase-phase plot for $20\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/Phase-Phase/Phase_phase_20.png}}
      \subfloat[Phase-phase plot for $30\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/Phase-Phase/Phase_phase_30.png}}
      
\end{multicols}

\begin{multicols}{3}
    \subfloat[Swingup with $40\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/theta_40pc1.png}}    
      \subfloat[Swingup with $50\%$ perturbation]{\includegraphics[width=1\linewidth]{images/NN_Pendulum/LTV/theta_50pc1.png}}
      \subfloat[Swingup with $60\%$ perturbation]{\includegraphics[width=1\linewidth]{images/NN_Pendulum/LTV/theta_60pc1.png}}
      \\
      \subfloat[Phase-phase plot for $40\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/Phase-Phase/Phase_phase_40.png}}
      \subfloat[Phase-phase plot for $50\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/Phase-Phase/Phase_phase_50.png}}
      \subfloat[Phase-phase plot for $60\%$ perturbation]{\includegraphics[width=\linewidth]{images/NN_Pendulum/LTV/Phase-Phase/Phase_phase_60.png}}    
\end{multicols}

\caption{{Benchmarking the performance of the nonlinear SINDY and MLP models with the LTV model on swing-up pendulum trajectories.}}
\vspace{-0.4cm}
\label{fig:LTV}
\end{figure*}

\subsubsection{Benchmarking for the Cartpole system}
Similarly, we generate the optimal trajectory and control for the modified Cartpole swingup task: Starting from the downward position of the pendulum ($\theta_0=180^\circ$) and the cart at rest, the cart needs to move such that the pendulum comes to rest at $\theta_T = 60^\circ$ within 30 time-steps. The training and testing data size and sampling methods remain the same. We train both the MLP model and SINDy on these data-points and generate the predictions to compare their performance against the LTV model. 

\begin{figure}[!htpb]

\begin{multicols}{2}
    %\hspace{1.4cm} 
      \subfloat[Cart position]{\includegraphics[width=\linewidth]{images/NN_Cartpole/swingup/Cartpole_1pc_x.png}}    
      \subfloat[Pendulum position]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/swingup/Cartpole_1pc_theta.png}}
      \\
      \subfloat[Cart Velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/swingup/Cartpole_1pc_xdot.png}}
      \subfloat[Pendulum angular velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/swingup/Cartpole_1pc_thetadot.png}}
      
\end{multicols}

\begin{multicols}{2}
    \subfloat[Cart position]{\includegraphics[width=\linewidth]{images/NN_Cartpole/swingup/Cartpole_5pc_x.png}}    
      \subfloat[Pendulum position]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/swingup/Cartpole_5pc_theta.png}}
      \\
      \subfloat[Cart Velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/swingup/Cartpole_5pc_xdot.png}}
      \subfloat[Pendulum angular velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/swingup/Cartpole_5pc_thetadot.png}}
          
\end{multicols}

\caption{{Benchmarking the performance of the nonlinear SINDY and MLP models with the LTV model on swing-up Cartpole trajectories.}}

\label{fig:LTV_Cartpolr}
\end{figure}

\subsection{Model Convergence}

In order to verify our theoretical analysis, we have to determine the convergence of the identified models. In order to do so, we sample trajectories from the same region of our dynamics, with different random seeds. The SINDY and MLP models are trained on these separate data samples, and we expect the dynamics learned to be consistent with one another if learning the same dynamics. From Fig.~\ref{fig:Convergence_SINDY}, we observe that the trajectories learned by each model begin to differ, with the difference increasing as we increase the scope of our neighborhood around the optimal trajectory.

\begin{figure}[!htpb]

\begin{multicols}{2}
    %\hspace{1.4cm} 
      \subfloat[Cart position]{\includegraphics[width=\linewidth]{images/NN_Cartpole/Sindy_seed/x_10pc1.png}}    
      \subfloat[Pendulum position]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/Sindy_seed/Theta_10pc1.png}}
      \\
      \subfloat[Cart Velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/Sindy_seed/xdot_10pc1.png}}
      \subfloat[Pendulum angular velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/Sindy_seed/Omega_10pc1.png}}
      
\end{multicols}

\begin{multicols}{2}
    \subfloat[Cart position]{\includegraphics[width=\linewidth]{images/NN_Cartpole/Sindy_seed/x_40pc1.png}}    
      \subfloat[Pendulum position]{\includegraphics[width=1\linewidth]{images/NN_Cartpole/Sindy_seed/Theta_40pc1.png}}
      \\
      \subfloat[Cart Velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/Sindy_seed/xdot_40pc1.png}}
      \subfloat[Pendulum angular velocity]{\includegraphics[width=\linewidth]{images/NN_Cartpole/Sindy_seed/Omega_40pc1.png}}
          
\end{multicols}

\caption{{Observing the convergence of the SINDY model learned on datasets with random initial seeds, with perturbations of $10\% U_{max}$ (a)-(d) and $40\% U_{max}$ (e)-(h) w.r.t. the optimal swingup trajectory.}}

\label{fig:Convergence_SINDY}
\end{figure}

==> Theory.tex <==
\section{Preliminaries}
\label{probform}
Consider the discrete-time nonlinear dynamical system:
\begin{equation}
    x_{t+1}=f(x_t, u_t),
\label{eq:dyn}
\end{equation}
where $x_t\in \mathbb{R}^{n_x}$ and $u_t\in \mathbb{R}^{n_u}$ correspond to the state and control vectors at time $t$. The optimal control problem is to find the optimal control policy $\pi^0=\{\pi^0_0, \pi^0_1 ... \pi^0_{T-1}\}$, that minimizes the cumulative cost:
\begin{align*}
    & \min_\pi J^\pi(x)=\sum_{t = 0}^{T-1} c_t(x_{t}, u_{t}) + c_T(x_T),% \\
    %&\text{Subject to:}\  x_{t+1}=f(x_t, u_t),
\end{align*}
subject to the dynamics above,
given some $x_0 = x$, and where $u_t=\pi_t^0(x_t)$, $c_t(\cdot)$ is the instantaneous cost function and $c_T(\cdot)$ is the terminal cost. We assume the incremental cost to be quadratic in control, such that $c_t(x_t,u_t)=l_t(x_t)+\frac{1}{2}u_t^T R u_t$.

In this work, we assume that we only have access to the input-output model of the dynamical system, wherein given the inputs $x$ and $u$, a black-box (computational) model generates the next state $x'=f(x,u)$.

% \vspace{-0.35cm}
\subsection{Model Structure} %For instance, these may be linear approximation architectures like SINDy, or nonlinear architectures such as (deep) neural networks. 
We consider three alternatives:
\begin{enumerate}
\item a ``global" linear in parameters approximation architecture with nonlinear basis functions ($f (x,u) \approx \sum_i c_i \psi_i(x,u)$), 
\item a ``global" nonlinear in parameters architecture, such as a (deep) neural network, ($f(x,u) \approx h(x,u;\theta)$), and 
\item a ``local" linear time varying (LTV) architecture ($\delta x_t = A_{t-1}\delta x_{t-1} + B_{t-1}\delta u_{t-1}$), linearized around a nominal trajectory $(\bar{x}_t,\bar{u}_t)$.
\end{enumerate}
The first two architectures estimate a ``global" model of the underlying dynamics while the third only finds a ``local perturbation" model of the dynamics. Since we are considering an optimal control problem, the ``local" model is an LTV approximation of the perturbation dynamics around the current estimate $(\bar{x}_t,\bar{u}_t)$ of the optimal trajectory, i.e., $\delta x_t = x_t - \bar{x}_t, \delta u_t = u_t -\bar{u}_t$. Moreover, these LTV models need to be recursively updated as the optimization proceeds (see Fig.~\ref{fig:optcontrol}(a)-(b)). In the case of the global approximators, in theory, such a model update is not required, since the approximate model should have global validity given enough training data.  
%The ``hope" is to be able to train these models with enough input-output data from the original black-box such that after training, we can obtain a cheap surrogate model to find the optimal control for the system.

For solving the optimal control problem using LTV models, we utilize the Iterative Linear Quadratic Regulator (ILQR) algorithm, which can be guaranteed to converge to the global optimum \cite{wang2021search}. A brief description of the ILQR Algorithm is given in the appendix.

%\subsection{The Need for Surrogate Modeling, and Comparison with Linear Time-Varying}
%\textcolor{blue}{A pertinent question in context with the work deals with the following: Why is there a need for surrogate modeling, when a black box is already available, and thus a `local' sampling-based approach can solve the optimal control problem? The issues with such an approach typically lie in computational complexity and scaling for larger-scale systems (\textit{e.g.} DNS simulations for the Navier-Stokes equation). For such systems, the computational complexity involved in even single-step evaluations of the black-box models is very high, thus making consistent sampling infeasible. Nonlinear surrogate modeling should, in turn, provide faster evaluations for such systems, while theoretically capturing the nonlinear characteristics present in the black-box models, hence providing a `global' estimator for the same.}

%\textcolor{blue}{One might also question why the data-intensive nature of nonlinear parametric estimators such as deep neural networks (with convergence guarantees known to be asymptotic at best) is an issue, when the sampling can be done in an offline fashion using the given black box.}
% \textcolor{blue}{Despite neural networks being known to be data-intensive, with convergence guarantees known to be asymptotic at best, one might question why it is an issue when doing offline computation with the black-box already given. }

%\textcolor{blue}{This is largely because solving the moment-estimation problem through nonlinear estimators requires samples that grow in a combinatorial-exponential fashion! Thus, for any reasonable estimate of the physical system, coupled with expensive simulations for systems, this approach becomes largely intractable. These techniques are also, in general, prone to high variances in their estimates, the reasons for which are explored in the subsequent sections.}

%\textcolor{blue}{Meanwhile, linear time-varying approximation, while being `local' in scope owing to the nature of its definition, implicitly solves the issue of the high-variance and ill-conditioning. Also, it has a significantly reduced sampling-complexity, of the order $O(n_x+n_u)$, while giving reliable models in the local neighbourhoods. }

\subsection{Data Generation and the Model Estimation Problem}

Let $f, g:\mathbb{R}\rightarrow \mathbb{R}$ be an infinitely smooth function, and $p(\cdot)$ be a p.d.f./sampling distribution on $\mathbb{R}$ from which training/ identification data is sampled. The inner product w.r.t. the distribution $p(\cdot)$ is defined as %$\langle f,g \rangle = \int_{-\infty}^{\infty} f(x)g(x)p(x)dx$.
\begin{equation*}
   \langle f,g \rangle = \int_{-\infty}^{\infty} f(x)g(x)p(x)dx. 
\end{equation*}

We are interested in approximating the function $f(\cdot)$ using a suitable architecture. For simplicity, we consider a scalar, control-free dynamical model $f(\cdot)$. Nonetheless, the results are generalized in a relatively straightforward fashion, while the issues inherent in the estimation problem come into sharp focus in the one dimensional setting.

\textbf{Linear.} Given a set of basis functions $\{\psi_0 ... \psi_M\}$, we want to approximate $f$ in the subspace spanned by $\Psi = \{\psi_0...\psi_M\}$, i.e., we want to find 
\begin{equation}
    \hat{f}=\sum_{i=0}^{M} \hat{c}_i \psi_i,
\end{equation}
such that $||f-\hat{f}||$ is minimized, where $||f||=\sqrt{\langle f,f \rangle}$ is the norm induced by the $p(.)$ weighted inner product above. Further, we want to find the number of samples $R$ required such that an $\varepsilon-$close approximation can be made to the true solution given we only have access to samples $(x^i,f(x^i))$ from the underlying distribution.

\textbf{Nonlinear.} Given a nonlinear approximation architecture $h(x,\theta)$, such as a (deep) neural network, we want to find the best approximation of $f$ in the approximation architecture, i.e. find $f^* = h(x,\theta^*)$ such that $||f-f^*||^2$ is minimized over all parameters $\theta \in \Theta \subseteq \Re^n$. Further, we want to approximate the number of samples to make an $\varepsilon-$close approximation based on only the samples $(x^i,f(x^i))$ from the underlying distribution.

%\begin{remark}
 %   In the following development, `linear case' refers to the linear in parameters approximation architecture, while `nonlinear case' refers to a nonlinear in parameters architecture.
%\end{remark}

\section{Convergence in the Model Estimation Problem}\label{truesec3}
In this Section, we characterize the solution to the model estimation problem posed above in the linear as well as nonlinear case and give estimates of the number of samples required/ sample complexity when solved in a data-based fashion.
\subsection{Linear Case}
We can get the answer to the linear question from the Projection Theorem in the Hilbert space $L_2(p)$ \cite{Courant-Hilbert}. 

The optimal $\hat{f}$ is such that $(f-\hat{f})\perp \psi_i \forall i=1,2...M$, owing to the Projection Theorem. Substituting $\hat{f} =\sum_{i=0}^M \hat{c}_i \psi_i$ leads to the Normal equations:
%\begin{equation}
 %   \mathcal{G}c^* = F\\
  %  \implies c^*=\mathcal{G}^{-1}F
%\end{equation}
%where $\mathcal{G}_{ij}= \langle \psi_i,\psi_j \rangle$, $F_i = \langle f,\psi_i \rangle$, $i,j = 1,2\cdots n$. %$\begin{bmatrix}<\psi_1,\psi_1> &<\psi_1,\psi_2>&\hdots &<\psi_1,\psi_n>\\ <\psi_2,\psi_1> &<\psi_2,\psi_2>&\hdots &<\psi_2,\psi_n> \\ \vdots & &\ddots \\ <\psi_n,\psi_1> &<\psi_n,\psi_2>&\hdots &<\psi_n,\psi_n>\end{bmatrix}$ is the corresponding Gram matrix and $F =$
%$\begin{bmatrix}
    %<f,\psi_1>\\ \vdots \\ <f,\psi_n>
%\end{bmatrix}$ is a vector containing the projections of $f$ along the directions $\{\psi_1,\psi_2... \psi_n\}$.
%This result implies that there exists a unique $f^*$ such that $||f-f^*||$ is minimized, given a linear approximation architecture, owing to the invertibility of $\mathcal{G}$ stemming from the linear independence of the basis $\{\psi_i\}$.
%The normal equations are:
\begin{align}
    \mathcal{G} \hat{C}_M &= F, \label{N}\\
    \mathcal{G}_{ij} &= \gamma_{ij} = \langle \psi_i, \psi_j \rangle, \quad i,j = 0, \dots, M, \label{eq:fij} \nonumber \\
    f_i &= \langle f, \psi_i \rangle 
         = \int f(x) \, \psi_i(x) \, p(x) \, dx
         = \mathbb{E}[f \, \psi_i],  \nonumber
\end{align}
where $\hat{C}_M= [\hat{c}_0, \cdots \, \hat{c}_M]'$, and $M$ is the order of the approximation.

Next, we assume that $p(x)$ is specified by an exploration parameter $\sigma$. For instance:
\begin{align}
    p(x) &\sim \mathcal{N}(x; 0, \sigma^2) \quad \text{(Gaussian)}, \nonumber \\
    p(x) &\sim U(x; -\sigma, \sigma) \quad \text{(Uniform)}. \nonumber
\end{align}
Thus, the functions $f_i(.)$ are a function of the parameter $\sigma$.

Next, let us assume that $f$ is exactly approximated in the basis set given an infinite number of basis functions, and define:
\begin{align}
    f(x) &= \sum_{k=0}^\infty c_k^* \, \psi_k(x), \\
    f_i(\sigma) &= \sum_{k=0}^\infty c_k^* \, \mathbb{E}[\psi_i \, \psi_k]
               \equiv \sum_{k=0}^\infty c_k^* \, \gamma_{i,k}(\sigma), \nonumber \\
    f_{i,M}(\sigma) &= \sum_{k \le M} c_k^* \, \gamma_{i,k}(\sigma), \nonumber\\
    \delta_{i,M}(\sigma) &= \sum_{k > M} c_k^*
    \gamma_{i,k}(\sigma). \nonumber \label{eq:delta}
\end{align}
Note the distinction between the coefficients $\hat{c}_k$ and $c_k^*$ and that $\hat{c}_k \rightarrow c_k^*$ as $M \rightarrow \infty$.\\

Next, we digress a little and have the following supporting development.
Let $g(\sigma)$ be an infinitely smooth function of the variable $\sigma \ge 0$, and further let  
\begin{align}
    g(\sigma) &= \sum_{k=0}^\infty g_k \, \zeta_k(\sigma). \nonumber
\end{align}

Define: 
\begin{align*}
    g_M(\sigma) = \sum_{k \le M} g_k \, \zeta_k(\sigma),\;
    \delta g_M(\sigma) = \sum_{k > M} g_k \, \zeta_k(\sigma). 
\end{align*}

\textbf{Definition:} The infinitely smooth function $g(\sigma)$ is said to have the \emph{Uniform Approximation (UA)} property with respect to the series of infinitely smooth functions $\{\zeta_k(\sigma)\}$ if  given any $M> 0$, and any $\varepsilon >0$, there exists $\sigma_M^{\varepsilon} > 0$ such that: $|\delta g_M(\sigma)| \leq \varepsilon |g_M(\sigma)|$, for any $\sigma \leq \sigma_M^{\varepsilon}$.

%\begin{align*}
 %   \lim_{\sigma \to 0} R_M(\sigma) &= 0, \\
 %   \lim_{\sigma \to \infty}R_M(\sigma) &= \infty, \, \text{for any } M > 0.
%\end{align*}
The above definition models the intuition that for an approximation scheme to be applicable, any $M^{th}$ order expansion of a function is sufficiently good in some suitable bounded region.
For instance, the U$\varepsilon$A is satisfied if the functions $\zeta_k(\sigma)$ are polynomials of degree $k$ and if the function $g(\sigma)$ has an infinite Taylor series expansion.\\

%\begin{lemma}  
%Given that the function $g(\sigma)$ has the SAP with respect to the set of basis functions $\{\zeta_k(\sigma)\}$, then for any $M > 0$, any $\varepsilon > 0$,  
%there exists $\sigma_M^\varepsilon$ such that for any $\sigma \le \sigma_M^\varepsilon$,
%\begin{align}
 %   |\epsilon_M(\sigma)| \le \varepsilon \, |g_M(\sigma)|.
%\end{align}
%\end{lemma}
%\begin{proof}  
%By definition, $g(\sigma)$,  
%$g_M(\sigma)$ and $\delta_M(\sigma)$ are all smooth functions.  
%This implies that  
%$
%    R_M(\sigma) = \frac{|\epsilon_M(\sigma)|}{|g_M(\sigma)|},
%$
%is continuous.  
%Since $\lim_{\sigma \to 0} R_M(\sigma) = 0$,  
%there exists a $\sigma_M^\varepsilon$ such that $R_M(\sigma) = \varepsilon$ for the first time at $\sigma = \sigma_M^\varepsilon$.  
%This, in turn, implies
%$
%    |\epsilon_M(\sigma)| \le \varepsilon \, |g_M(\sigma)|, \, \text{for} \,\sigma \le \sigma_M^\varepsilon.%
%$
%\end{proof}

%Next, we can state the following result.  
%Consider the normal equations \eqref{N}.  
%Let  
%$
 %   f(x) = \sum_{k=0}^\infty c_k^* \, \psi_k(x),
%$
%and let the $M$-th order approximation $\hat{f}(\sigma)$ resulting from the Normal equations be  
%$
 %   \hat{f}(x) = \sum_{k=0}^M \hat{c}_k \, \psi_k(x).
%$

\begin{lemma}  \label{e-lemma}
Let the functions $f_i(\sigma)$ have the UA property with respect to the sequence of infinitely smooth functions $\{\gamma_{i,k}(\sigma)\}$ for any $i$.  
Then, there exists a $\bar{\sigma}$ such that for all $\sigma \le \bar{\sigma}$, 
\begin{align}
    |\delta_{i,M}(\sigma)| \le \varepsilon \, |f_{i,M}(\sigma)|, \quad \forall j. 
\end{align}
\end{lemma}
\begin{proof}  
Since $f_i(\sigma)$ has the UA property, for each $i$ there exists $\sigma_{i,M}^{\varepsilon}$  
such that for all $\sigma \le \sigma_{i,M}^{\varepsilon}$,  
$
    |\delta_{i,M}(\sigma)| \le \varepsilon \, |f_{i,M}(\sigma)|.
$
Take  
\begin{align}
    \bar{\sigma} = \min_i \sigma_{i,M}^{\varepsilon}, \nonumber
\end{align}
then it follows that  for any $i$,
\begin{align}
    |\delta_{i,M}(\sigma)| \le \varepsilon \, |f_{i,M}(\sigma)|, \quad \sigma \le \bar{\sigma}. \nonumber
\end{align}
\end{proof}
Let  
\begin{align}
    C_M^* &= 
    \begin{bmatrix}
        c_0^* \\ \vdots \\ c_M^*
    \end{bmatrix},
    &
    \hat{C}_M &=
    \begin{bmatrix}
        \hat{c}_0 \\ \vdots \\ \hat{c}_M
    \end{bmatrix}.
\end{align}
\begin{proposition}  \label{ME_acc}
Given the sampling parameter $\sigma \le \bar{\sigma}$,
\begin{align}
    \| C_M^* - \hat{C}_M \| &\le \kappa(\mathcal{G}) \, \| C_M^* \| \, \varepsilon,
\end{align}
where  
$
    \kappa(\mathcal{G}) = \| \mathcal{G} \| \, \| \mathcal{G}^{-1} \|
$
is the condition number of the Gram matrix, and $\| \cdot \|$ is the matrix norm induced by the vector norm $||.||$.
\end{proposition}

\begin{proof}  
Consider the model estimation equation:
\begin{align}
    \mathcal{G} \hat{C}_M &= F(\sigma) \equiv
    \begin{bmatrix}
        f_0(\sigma) \\
        \vdots \\
        f_M(\sigma)
    \end{bmatrix}, \nonumber
\end{align}
However,
$
    f_i(\sigma) = f_{i,M}(\sigma) + \delta_{i,M}(\sigma).
$

Note that:
\begin{align}
    F_M(\sigma) &\equiv
    \begin{bmatrix}
        f_{0,M}(\sigma) \\
        \vdots \\
        f_{M,M}(\sigma)
    \end{bmatrix}
    =
    \mathcal{G} C_M^*. \nonumber
\end{align}

Hence, defining:
\begin{align*}
    \Delta_M(\sigma) = 
    \begin{bmatrix}
    \delta_{0,M} (\sigma)\\
    \vdots\\
    \delta_{M,M} (\sigma)
    \end{bmatrix}
\end{align*}
it follows that:
\begin{align}
    \mathcal{G} \, \hat{C}_M &= \mathcal{G} \, C_M^* + \Delta_M, \\
    \hat{C}_M - C_M^* &= \mathcal{G}^{-1} \Delta_M. \nonumber
\end{align}

Therefore:
\begin{align}
    \| \hat{C}_M - C_M^* \| &\le \| \mathcal{G}^{-1} \| \, \| \Delta_M \|, \nonumber \\
    &\le \| \mathcal{G}^{-1} \| \, \varepsilon \, \| {F}_M \| 
    \quad \text{(by Lemma 2)}, \nonumber \\
    &\le \| \mathcal{G}^{-1} \| \, \| \mathcal{G} \| \, \| C_M^* \| \, \varepsilon 
    = \kappa(\mathcal{G}) \, \| C_M^* \| \, \varepsilon. \nonumber
\end{align}
\end{proof}
\begin{remark}
    In order to make an $\varepsilon$-close approximation of a function to $M^{th}$ order by sampling, we need a certain exploration $\bar{\sigma}$ that is dependent on all the moments $f_i(\sigma) = \mathbb{E}[f\psi_i]$, $i=0,1,2,\cdots M$. Furthermore, the accuracy of the approximation is critically dependent on the conditioning $\kappa(\mathcal{G})$ of the Gram matrix.
\end{remark}

Next, we assume that we have access only to the data-points $(x^k, f(x^k)), k=1,2...R$, where the samples are drawn from the sampling distribution, $x^k\sim p(\cdot)$, independently. 
Given the sample set $(x^k, f(x^k))$, we approximate:
\begin{equation}
\label{eq: Leastsquares}
    f(x^k) \approx \sum_{j=1}^M c_i \psi_i (x^k)~ \forall~ k=1,2...R.
\end{equation}
%\begin{bmatrix}
    %f(x^1)\\
    %\vdots\\
    %f(x^R)
%\end{bmatrix}$. 
The least squares solution to Eq.~\ref{eq: Leastsquares} is given by:
\begin{equation}
\label{eq: Leastsquares solution}
    \hat{C}^R_M = (\underbrace{{\Psi}^{R'}{\Psi}^R}_{\mathcal{G}^R})^{-1} {\Psi}^{R'} F^R,
\end{equation}

 where, 
 \begin{align*}
     ({\Psi}^{R'}{\Psi}^R)_{ij}=\sum_{k=1}^R \psi_i(x^k)\psi_j(x^k) \equiv R\gamma_{ij}^R, \\
   ({\Psi}^{R'}F^R)_i = \sum_{k=1}^R \psi_i(x^k)f(x^k) \equiv Rf_i^R.
 \end{align*}
 
   
 Owing to the law of large numbers \cite{gnedenko}, we have: %$\frac{1}{R} \sum_{i=1}^R \psi_k(x^i)\psi_l(x^i)\rightarrow \int \psi_k(x)\psi_l(x)p(x)dx=\langle \psi_k,\psi_l \rangle$, and $\frac{1}{R} \sum_{i=1}^R \psi_k(x^i)f(x^i)\rightarrow \int \psi_k(x)f(x)p(x)dx=\langle \psi_k,f \rangle$,
\begin{equation*}
    \frac{1}{R} \sum_{k=1}^R \psi_i(x^k)\psi_j(x^k)\rightarrow \int \psi_i(x)\psi_j(x)p(x)dx=\underbrace{\langle \psi_i,\psi_j\rangle}_{\gamma_{ij}},
\end{equation*}
and
\begin{equation*}
    \frac{1}{R} \sum_{k=1}^R \psi_i(x^k)f(x^k)\rightarrow \int \psi_i(x)f(x)p(x)dx=\underbrace{\langle \psi_i,f\rangle}_{f_i} ,
\end{equation*}
as $R\rightarrow\infty$. This implies that %$\Bar{C}^R=(\underline{\Psi}^{R'} \underline{\Psi}^R)^{-1}(\underline{\Psi}^{R'}F^R) = (\frac{1}{R}\underline{\Psi}^{R'} \underline{\Psi}^R)^{-1}(\frac{1}{R}\underline{\Psi}^{R'}F^R) \rightarrow(\mathcal{G})^{-1}F \text{ as } R\rightarrow\infty$. 
\begin{align*}
    %\implies
    \hat{C}^R_M&=({\Psi}^{R'} {\Psi}^R)^{-1}({\Psi}^{R'}F^R)\\
    &=(\frac{1}{R}{\Psi}^{R'} {\Psi}^R)^{-1}(\frac{1}{R}{\Psi}^{R'}F^R)\\
    &\rightarrow(\mathcal{G})^{-1}F = \hat{C}_M \text{ as } R\rightarrow\infty.
\end{align*}
Therefore, the data-based solution converges to the true solution of the Normal Equation, as $R\rightarrow \infty$.\\
Albeit the Least-Squares estimate converges to the true solution of the Normal equation in the limit, we would like to find an estimate of the samples $R$ required for some given error level $\epsilon$. In this regard, we first present the following facts.

Let $g(x)$ be a function of the random variable $x$. Then $\Bar{g}\equiv E[g(x)]=\frac{1}{R}\sum_{j=1}^{R}g(x^j)$ as $R\rightarrow\infty$. Furthermore, if $R$ is large enough, due to the Central Limit Theorem \cite{gnedenko}, $\Bar{g}^R \equiv \frac{1}{R}\sum_{k=1}^{R}g(x^k) = N(\Bar{g}, \frac{\sigma_g^2}{R})$,
% \begin{equation*}
%     \Bar{g}^R \equiv \frac{1}{R}\sum_{i=1}^{R}g(x^i) = N(\Bar{g}, \frac{\sigma_g^2}{R}),
% \end{equation*}
where $\sigma_g^2= Var[g(x)]$, and $N(\mu,\sigma^2)$ is a normal random variable with mean $\mu$ and variance $\sigma^2$. Next, the r.v. $\frac{\bar{g}^R - \bar{g}}{\sigma_g/ \sqrt{R}} \sim N(0,1)$. Thus:
\begin{align}
    Prob(|\bar{g}^R - \bar{g}|> \epsilon) = 1- \Phi(\frac{\epsilon\sqrt{R}}{\sigma_g^2}),
\end{align}
where $\Phi(a)$ (termed the erf) represents the probability that a standard Gaussian r.v. z, i.e., $z\sim N(0,1)$, takes values $|z|<a$.\\
\\ %Then, we can give the error estimate %$Prob(|\Bar{g}^R-\Bar{g}|>\epsilon)\leq \frac{\sigma_g}{\sqrt{2\pi R}} e^{\frac{-\epsilon^2R}{\sigma_g^2}}$.
%\begin{equation*}
 %   Prob(|\Bar{g}^R-\Bar{g}|>\epsilon)\leq \frac{\sigma_g}{\sqrt{2\pi R}} e^{\frac{-\epsilon^2R}{\sigma_g^2}}.
%\end{equation*}
% \begin{equation}
%     Prob(|\Bar{g}^R-\Bar{g}|>\epsilon)\leq \frac{\sigma_g}{\sqrt{2\pi R}} e^{\frac{-\epsilon^2R}{\sigma_g^2}}.
% \end{equation}
Recall that $f_i = \langle \psi_i, f \rangle$, and thus:
\begin{align*}
    f_i^R \equiv \frac{1}{R}\sum_{k=1}^R \psi_i(x^k)f(x^k)
    \sim N(f_i,\frac{\nu_i^2}{R})
\end{align*}

% \begin{equation*}
%     f_k^R \sim N(f_k,\frac{\sigma_k^2}{R})
% \end{equation*}
where $\nu_i^2=Var[\psi_i(x)f(x)]$. Further, recall that the elements of the Gram matrix are $\gamma_{ij}=\langle \psi_i,\psi_j \rangle$, and that $\frac{1}{R}\underline{\Psi}^{R'}\underline{\Psi}^R \rightarrow \mathcal{G}$ as $R\rightarrow \infty$. Thus, %$\mathcal{G}_{kl}^R \equiv \frac{1}{R}\sum_{i=1}^R \psi_k(x^i)\psi_l(x^i) \sim N(\mathcal{G}_{kl}, \frac{\sigma_{kl}^2}{R})$,
\begin{equation*}
    \gamma_{ij}^R \equiv \frac{1}{R}\sum_{k=1}^R \psi_i(x^k)\psi_j(x^k) \sim N(\gamma_{ij}, \frac{\nu_{ij}^2}{R}),
\end{equation*}
where $\nu_{ij}^2= Var[\psi_i(x)\psi_j(x)]$.
Then, it follows from the development above that:
\begin{align*}
    Prob(|f_i^R-f_i|>\epsilon)= 1-\Phi(\frac{\epsilon \sqrt{R}}{\nu_i}),\\
    Prob(|\gamma_{ij}^R-\gamma_{ij}|>\epsilon)= 1-\Phi(\frac{\epsilon \sqrt{R}}{\nu_{ij}}).
\end{align*}

The above development may now be summarized in the following result.\\

\begin{proposition}\label{prop2}
The solution of the data-based Least-Squares problem (Eq.~\ref{eq: Leastsquares solution}) $\hat{C}^R_M\rightarrow \hat{C}_M$, the solution of the Normal Equation, as $R\rightarrow\infty$, in the mean square sense. Furthermore, $f_i^R \sim N(f_i, \frac{\nu_i^2}{R})$, $\gamma_{ij}^R\sim N(\gamma_{ij}, \frac{\nu_{ij}^2}{R})$, and $ Prob(|f_i^R-f_i|>\epsilon)= 1-\Phi(\frac{\epsilon \sqrt{R}}{\nu_i})$, $ Prob(|\gamma_{ij}^R-\gamma_{ij}|>\epsilon)= 1-\Phi(\frac{\epsilon \sqrt{R}}{\nu_{ij}})$.
\end{proposition}
Suppose, now we want a failure probability of at most $\delta$ that each $|\gamma_{ij}^R - \gamma_{ij}|> \epsilon,\, |f_i^R - f_| > \epsilon$. Then, the number of samples required for the $f_i^R$ to reach this confidence level is:
\begin{align*}
    R_i = \nu_i^2 \frac{p^2(\delta)}{\epsilon^2},
\end{align*}
and the number of samples required for the $\gamma_{ij}^R$ is:
\begin{align*}
    R_{ij} = \nu_{ij}^2 \frac{p^2(\delta)}{\epsilon^2},
\end{align*}
where $p(\delta) = \Phi^{-1}(1- \delta)$. Let:
\begin{align}\label{sample_C}
    R = \max\left( \max_i R_i, \max_{i,j} R_{ij}\right).
\end{align}
Let $\mathcal{G}^R = \mathcal{G} + \delta \mathcal{G}^R$ and $F^R = F+ \delta F^R$. Hence, if we set the number of samples $R$ as above, then we have, with probability at least $1-(M+ M^2)\delta$:
    \begin{align}
        ||\delta F^R|| \leq \epsilon, \, ||\delta \mathcal{G}^R||\leq M\epsilon, 
    \end{align}
    where $||.||$ is the max-norm or the matrix norm induced by the max-norm depending on the argument being a vector or a matrix.\\
     Then, the R-sample solution, after ignoring the second and higher order terms of the small variables $\delta F^R$ and $\delta \mathcal{G}^R$, can be written as:
    \begin{align*}
        C_M^R &= (\mathcal{G} + \delta \mathcal{G}^R)^{-1}(F + \delta F^R),\\
        &\approx \mathcal{G}^{-1} F - \mathcal{G}^{-1}\delta F^R - \mathcal{G}^{-1}\delta \mathcal{G}^R\mathcal{G}^{-1} F.
    \end{align*}
    Noting that $\hat{C}_M = \mathcal{G}^{-1} F$, it follows that:
    \begin{align*}
        C_M^R - \hat{C}_M = - \mathcal{G}^{-1}\delta F^R - \mathcal{G}^{-1}\delta \mathcal{G}^R\mathcal{G}^{-1} F,
    \end{align*}
    and hence,
    \begin{align*}
        ||C_M^R - \hat{C}_M|| &\leq ||\mathcal{G}^{-1}||||\delta F^R|| + ||\mathcal{G}^{-1}||^2||F|| ||\mathcal{\delta G}^R||,\\
        &\leq K_G\epsilon + K_G^2K_FM \epsilon \equiv \mathcal{C} \epsilon,
    \end{align*}
where $||\mathcal{G}^{-1}|| = K_G, \, ||F|| = K_F,\, \mathcal{C} = K_G + K_G^2 K_F M$.\\
However, from Proposition 1, we know that $||C_M^* - C_M|| \leq \kappa(\mathcal{G})||C_M^*|| \varepsilon$. Therefore, it follows that the error between the R-sample solution and the true solution satisfy:
\begin{align*}
    ||C_M^R - C_M^*|| \leq \mathcal{C}\epsilon + \kappa(\mathcal{G})||C_M^*||\varepsilon.
\end{align*}
The development above can be summarized as the following result.\\
\begin{proposition}
    Let $R$ be chosen as in Eq. \ref{sample_C}. Then, with probability at least $1-(M+M^2)\delta$, the R-sample estimate $C_M^R$ satisfies: \begin{align*}
    ||C_M^R - C_M^*|| \leq \mathcal{C}\epsilon + \kappa(\mathcal{G})||C_M^*||\varepsilon,
    \end{align*}
    where  $||\mathcal{G}^{-1}|| = K_G, \, ||F|| = K_F,\, \mathcal{C} = K_G + K_G^2 K_F M$, $||.||$ is the max-norm when applied to vectors, and the max-induced matrix norm when applied to matrices. The error parameters $\varepsilon$ and $\epsilon$ were defined in Lemma \ref{e-lemma} and Proposition \ref{prop2}.\\
    \end{proposition}
\begin{remark}
 The above analysis suggests that given sufficient samples, the data-based solution can be a good approximation of the true solution given sufficiently small $\epsilon \text{and} \,\varepsilon$. However, note that the sample complexity for the error to be below level $\epsilon$ with high confidence $(1-\delta)$ is critically dependent on the variances $\nu_i^2$ and $\nu_{ij}^2$. Furthermore, the error in the solution $||C_M^R - C_M^*||$ is dependent on the conditioning $\kappa(\mathcal{G})$ of the underlying Gram matrix. 
\end{remark}

\subsection{Nonlinear Case}
Given the nonlinear approximation architecture, one has to solve the least-squares problem %$\theta^* = \min_\theta ||f-h(x,\theta)||^2$.
\begin{equation*}
    \theta^* = \min_\theta \frac{1}{2}||f-h(x,\theta)||^2.
\end{equation*}
This may be solved using a suitable optimization algorithm such as gradient descent. Let $J(\theta)=\frac{1}{2}||f-h(x,\theta)||^2=\int (f-h(x,\theta))^2 p(x)dx$. This implies that %$\frac{\partial J}{\partial \theta} = -2\int (f-h(x,\theta))h_\theta (x,\theta)p(x)dx$, 
\begin{equation*}
    \frac{\partial J}{\partial \theta} = -\int (f-h(x,\theta))h_\theta (x,\theta)p(x)dx,
\end{equation*}
where $h_\theta(x,\theta)=\frac{\partial h(x,\theta)}{\partial \theta}$. 

Then, we can set up the gradient descent recursion %$\theta_{t+1} = \theta_t - \gamma \frac{\partial J}{\partial \theta}\Bigg|_{\theta_t}$,
\begin{equation*}
    \theta_{t+1} = \theta_t - \gamma_t \frac{\partial J}{\partial \theta}\Bigg|_{\theta_t},
\end{equation*}
where $\theta_t \rightarrow\theta^*$ s.t. $\frac{\partial J}{\partial \theta}|_{\theta^*}=0$, given $\gamma_t \rightarrow 0$ and $\sum_t \gamma_t = \infty$ (see Ch. 3, Prop. 3.5 in \cite{NDP}). Note, however, that, unlike the linear case, there is no guarantee that the algorithm converges to the global minimum.
Moreover, for a local minimum $\theta^*$, $\langle \Delta^*,H_k^* \rangle = 0$, for all $k = 1,2 \cdots n$, where $\Delta^*(x) = f(x) - h(x,\theta^*),$ and $H^*_k = \frac{\partial h}{\partial \theta_k}|_{\theta^*}$, owing to the necessary condition above, analogous to the Projection Theorem in the linear case.\\

Next, we consider the data-driven estimation problem for the nonlinear parametrization. Given the approximation architecture $h(x,\theta)$, parameterized non-linearly by $\theta$, define $[F^R -H^R(\theta)]_j=f(x^j)-h(x^j,\theta)$ for $j=1,2...R$.
% \begin{bmatrix}
%         f(x^1)\\ \vdots \\ f(x^R)
%     \end{bmatrix} - \begin{bmatrix}
%         h(x^1,\theta)\\ \vdots \\ h(x^R, \theta)
%     \end{bmatrix}$.
% \begin{align*}
%     & F^R -H^R(\theta)=\begin{bmatrix}
%         f(x^1)\\ \vdots \\ f(x^R)
%     \end{bmatrix} - \begin{bmatrix}
%         h(x^1,\theta)\\ \vdots \\ h(x^R, \theta)
%     \end{bmatrix}.
% \end{align*}
Let us define our cost function $J^R(\theta)=||F^R-H^R(\theta)||^2= \frac{1}{2R}\sum_{j=1}^R (f(x^j)-h(x^j,\theta))^2$. Thus, we have the cost-gradient %$\frac{\partial J^R(\theta)}{\partial \theta}=- \frac{1}{R}\sum_{i=1}^R(f(x^i)-h(x^i,\theta))\frac{\partial h(x^i,\theta)}{\partial \theta}$.
\begin{equation*}
    \frac{\partial J^R(\theta)}{\partial \theta}=- \frac{1}{R}\sum_{j=1}^R(f(x^j)-h(x^j,\theta))\frac{\partial h(x^j,\theta)}{\partial \theta}.
\end{equation*}
From the Law of Large Numbers, we have $\frac{\partial J^R}{\partial \theta}\rightarrow \frac{\partial J}{\partial \theta}$ as $R\rightarrow \infty$. Thus, as the number of samples becomes large, the gradient estimate becomes arbitrarily accurate and the gradient descent algorithm is guaranteed to converge to a stationary point of the cost function. In particular, the following result holds. Let:
\begin{align*}
    \Delta(x) = f(x) - h(x,\theta), \; H^i(x) = \frac{\partial{h}}{\partial \theta_i},\\
    \mathrm{Var}[\Delta(x) H^i(x)] = \mu_i^2.
\end{align*}
\begin{proposition}
Given the step size parameters $\gamma_t$ satisfy $\sum_t \gamma_t = \infty, \; \sum_t \gamma_t^2 < \infty$ and the variances are uniformly bounded $\mu_i^2 < K< \infty$ for all $\theta$, the stochastic gradient descent sequence: $\theta_{t+1} = \theta_t - \gamma_t \frac{\partial J^R}{\partial \theta}$ converges to $\theta^*$ such that $\frac{\partial J}{\partial \theta}|_{\theta^*} = 0$, for any finite $R$.
\end{proposition}
\begin{proof}
    Let $\mathcal{F}^t$ denote the history of the algorithm till time $t$. Write $\frac{\partial J^R}{\partial \theta}|_{\theta_t} = \frac{\partial J}{\partial \theta}|_{\theta_t} + w_t$. Then, it follows due to the unbiased nature of the estimate that $\mathrm{E}[w_t/ \mathcal{F}^t] = 0$.  and $\mathrm{E}[||w_t||^2/ \mathcal{F}_t] \leq \frac{nK}{R} < \infty$, uniformly for all $t$. Therefore, the sequence $\theta_t$ is guaranteed to converge to a stationary point of the function $J(.)$ (Prop. 4.1, \cite{NDP}).
\end{proof}

Further, we can give sample complexity bounds for the error in the gradient estimate analogous to the linear case. Let:
\begin{align*}
    \nabla_iJ = \frac{\partial J}{\partial \theta_i},\; \nabla_i^R J = \frac{\partial J^R}{\partial \theta_i}.
\end{align*}
Then, due to the Central limit theorem, given $R$ is is large enough: $\nabla_i^RJ \sim \mathcal{N}(\nabla_iJ, \mu_i^2)$. \\
Thus, for $P(|\nabla_i^RJ - \nabla_i J|> \epsilon|) < \delta$, the number of samples required is:
\begin{align}\label{sample_grad}
    R_i = \mu_i^2 \frac{p^2(\delta)}{\epsilon^2}.
\end{align}
Hence, given $R = \max_i R_i$, with probability at least $(1-n\delta)$, $|\Delta_i^R J - \Delta_i J| < \epsilon$, for all $i=1,2,\cdots n$.\\

\begin{remark}
    There exists work that establishes the universal approximation properties of neural networks, both in the bounded depth and arbitrary width case \cite{NN_UA1,NN_UA2}, and more recently, in the bounded width and arbitrary depth case \cite{NN_UA3,NN_UA5,NN_UA4}. However, these are existence results and the actual training of these networks from data requires approaches such as backpropagation for which there are relatively few guarantees beyond convergence to a stationary point using stochastic gradient descent as outlined above.  The fundamental issue is that albeit there may be a unique parameter value that minimizes the cost, gradient descent cannot be expected to converge to that value. Further, as the size of the network is increased (either depth/ width), is there a unique or are there multiple parameter values that converge to the function being approximated, and if so, is there any guarantee that gradient descent via backpropagation can converge to any of these parameter values? These are open questions in the literature and beyond the scope of this paper, and thus, we do not provide a data-based approximation result such as Proposition 3 in the linear case. Nonetheless, in what follows, we will show that ill-conditioning and variance affect the training process adversely if approximating a function over a large domain/ high order, and consequently,  there is no guarantee regarding the convergence of the parameter estimates beyond the fact that they converge to a stationary point of the cost. Further, even with the same dataset, owing to the ill-conditioning and variance, gradient descent cannot be expected to converge to the same stationary point over multiple different runs.
\end{remark}
\section{Variance and Ill-Conditioning in the Model Estimation Problem}\label{sec_var_illcon}
In this Section, we shall show that the data-based solution suffers from very high variance as well as severe ill-conditioning if approximating over a large domain. %Note that $(\frac{1}{R}\underline{\Psi}^{R'}F^R)_i= f_i^R$ and $(\frac{1}{R}\underline{\Psi}^{R'}\underline{\Psi}^{R})_{ij}=\mathcal{G}_{ij}^R$, where $i,j=1,2...N$.
% \begin{bmatrix}
%     f_1^R\\ \vdots \\ f_N^R
% \end{bmatrix}$ and $\frac{1}{R}\underline{\Psi}^{R'}\underline{\Psi}^{R}= \begin{bmatrix}
%     \mathcal{G}_{11}^R &\hdots &\mathcal{G}_{1N}^R\\
%     \vdots & &\vdots\\
%     \mathcal{G}_{N1}^R &\hdots &\mathcal{G}_{NN}^R
% \end{bmatrix}$.

In order to make an approximation of the function $f(.)$ over a large domain, one has to sample with a large enough exploration parameter $\sigma$ as well as expand to a high enough order $M$. This, in turn, leads to two issues:

\textbf{Variance.} $\mathrm{Var}(f\psi^i) = \nu_i^2$ and $\mathrm{Var}(\psi_i\psi_j) = \nu_{ij}^2$ grows combinatorially-exponentially in the order $M$ and the size of the sampled domain $\sigma$.\\
\textbf{Ill-Conditioning.} The elements of the Gram matrix $\mathcal{G}_{ij}$ are exponentially-combinatorially different, leading to severe ill-conditioning.

As mentioned previously, the data based solution may be written as:
\begin{equation}
    \hat{C}^R_M=(\underline{\Psi}^{R'}\underline{\Psi}^{R})^{-1}\underline{\Psi}^{R'}F^R = (\mathcal{G}+\delta G^R)^{-1}(F+\delta F^R), \label{ill-cond}
\end{equation} 
where $\mathcal{G}$ and $F$ are the true Gram matrix and projections of $f$ on the basis vectors respectively. If the approximation order $M$ is high, the variance in the errors $\delta G^R$ and $\delta F^R$ is very large, and $\mathcal{G}$ is ill-conditioned, and thus, the data-based solution $\hat{C}^R_M$ is bound to have a large variance, and also be sensitive to small variations owing to the ill-conditioning. In the following development, we will characterize the variance in the estimates for some common choices of sampling distributions and generic basis functions.\\

\begin{remark}
    We note that the ill-conditioning is a feature of the problem formulation and is due to the high order approximation over a large domain. In addition, the variance stems from the data-based solution to the problem. 
\end{remark}

\subsection{Linear Case}
We have seen that the optimal estimates $\hat{C}_M$ and $C_M^*$ are $\varepsilon$-close (Proposition 2).  
Furthermore, as $R \to \infty$, we have shown that the data-based estimate $\hat{C}_M^R \to \hat{C}_M$.

Next, we need to characterize the variance of the data-driven solution:
\begin{align}
    \mathcal{G}^R \, \hat{C}_M^R &= (\Psi^R)' F^R,
\end{align}
where
$
    (\Psi^R)' \Psi^R = \mathcal{G}^R.
$

Noting that 
\begin{align}
   [ (\Psi^R)' f^R]_i &\to \mathbb{E}[f \, \psi^i], \nonumber
\end{align}
we need to find the mean $f_i$ and the variance $\nu_i^2$ of the variable $f \, \psi^i$.
Further,
\begin{align}
    (\Psi^R)' \Psi^R &\to \mathcal{G} = [ \gamma_{ij}(\sigma) ] = \left[ \mathbb{E}[\psi_i \, \psi_j] \right], \nonumber
\end{align}
so we need to find the mean $\gamma_{ij}$ and the variance of the random variable $\psi_i \, \psi_j$.

Define:
\begin{align}
    \mathbb{E}\left[ x^k \right] &= B_k \, \sigma^k. \\
    \text{Note that } &\text{if the variable $x$ is Gaussian, i.e., } x \sim \mathcal{N}(0, \sigma^2): \nonumber \\
    B_k &= 
    \begin{cases}
        \left( \frac{k}{2} - 1 \right)!!, & \text{if $k$ even}, \\
        0, & \text{if $k$ odd}.
    \end{cases}
\end{align}

\begin{align}
\text{Uniform: } U(-\sigma, \sigma), \quad 
B_k =
\begin{cases}
    \frac{1}{k+1}, & \text{if $k$ odd}, \\
    0, & \text{if $k$ even}.
\end{cases}
\end{align}
%\\[1em]

\begin{align}
\text{Also, let:} \quad
f(x) &= \sum_k \frac{F_k}{k!} x^k, 
\psi^i(x) &= \sum_m \frac{\beta_m^i}{m!} x^m, \nonumber
\end{align}
the Taylor expansions of the functions $f$ and $\psi^i$ respectively.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma} \quad 
The mean $f_i(\sigma)$ and the variance $\nu_i^2(\sigma)$ of the r.v. $f \psi^i$ is given by: 
\begin{align*}
\mathbb{E}[f\psi^i]&=f_i(\sigma) = \sum_{m,n} \frac{\beta^i_m F_n}{m! \, n!} \, B_{n+m} \, \sigma^{n+m}, \\[0.5em]
\mathrm{Var}(f \psi^i) &= \nu_i^2(\sigma) \\
&= \sum_{m,n,p,k} \frac{F_n F_k \beta^i_m \beta^i_p}{m! \, n! \, p! \, k!} \\
&\times \left( B_{n+m+p+k} - B_{n+m} B_{p+k} \right) \sigma^{n+m+p+k}.
\end{align*}
\end{lemma}


\begin{proof} 
\begin{align*}
f\psi^i = \sum_{m,n} \frac{F_n \beta^i_m}{m! \, n!} x^{n+m}. 
\end{align*}
Thus,
\begin{align*}
f_i(\sigma) = \mathbb{E}[f \psi^i] 
&= \sum_{m,n} \frac{F_n \beta^i_m}{m! \, n!} \mathbb{E}[x^{n+m}]\\
&= \sum_{m,n} \frac{F_n \beta^i_m}{m! \, n!} B_{n+m} \sigma^{n+m}.
\end{align*}
Similarly,
\begin{align*}
\nu_i^2 &= \mathrm{Var}(f \psi^i) 
= \mathbb{E} \big[ (f \psi^i - f^i)^2 \big] \\
&= \sum_{m,n,p,k} \frac{F_n \beta^i_m F_k \beta^i_p}{m! \, n! \, p! \, k!} 
\left[ \mathbb{E}[x^{n+m+p+k}] - \mathbb{E}[x^{n+m}] \mathbb{E}[x^{p+k}] \right] \\
&= \sum_{m,n,p,k} \frac{F_n F_k \beta^i_m \beta^i_p}{m! \, n! \, p! \, k!} 
\left( B_{n+m+p+k} - B_{n+m} B_{p+k} \right) \sigma^{n+m+p+k}.
\end{align*}
%\end{align}
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

By a similar development, we have the following result for the Gram matrix element  $(\psi_i \psi_j)$.\\
\begin{corollary} The mean $\gamma_{ij}(\sigma)$ and the variance $\nu_{ij}^2(\sigma)$ of the r.v. $\psi_i \psi_j$ are given by:
\begin{align*}
\gamma_{ij}(\sigma) &= \sum_{m,n} \frac{\beta^i_m \beta^j_n}{m! \, n!} \, B_{n+m} \, \sigma^{n+m}, \\[0.5em]
\nu_{ij}^2(\sigma)  &= \sum_{m,n,p,k} \frac{\beta^i_m \beta^j_n \beta^i_p \beta^j_k}{m! \, n! \, p! \, k!} \\
&\times\left( B_{n+m+p+k} - B_{n+m} B_{p+k} \right) \sigma^{n+m+p+k}.
\end{align*}
\end{corollary}

\textbf{Variance:}  
Note that the variance of $f \psi^i$ is an infinite sum over $m,n,p,k$. In general, this sum is difficult to evaluate. Thus, in order to get an idea about at least the order of the variance in an easily comprehensible form, assume that the maximum of the summand when $m=n=p=k$ occurs at some $N_i$. 
Then, using Lemma 2 and Corollary 1, it follows that:
\begin{align} \label{varianceF}
\nu_i^2=\mathrm{Var}(f \psi^i) \gtrapprox  O \left( \frac{B_{4N_i} - B_{2N_i}^2}{(N_i!)^4} \sigma^{4N_i} \right).
\end{align}
Similarly, the variance of $\psi_i\psi_j$ is an infinite sum and suppose that the maximum of the summand when $m=n=p=k$, occurs for some $L_{ij}$, then:
\begin{align} \label{varianceG}
\nu_{ij}^2=\mathrm{Var}(\psi^i \psi^j) \gtrapprox  O \left( \frac{B_{4L_{ij}} - B_{2L_{ij}}^2}{(L_{ij}!)^4} \sigma^{4L_{ij}} \right).
\end{align}

\textbf{Sample Complexity Revisited:}
    Using Proposition 3, it can be seen that the number of samples required such that $|f_i^R -f_i| > \epsilon$, where recall that $f_i^R$ is the R-sample average estimate of the mean $f_i$, with probability at most $\delta$ is given by:
    \begin{align}\label{Fsample}
        R_i \gtrapprox O\left(\frac{\nu_i^2}{\epsilon^2}p^2(\delta)\right) = O\left(\frac{B_{4N_i} - B_{2N_i}^2}{(N_i!)^4}\sigma^{4N_i} \frac{p^2(\delta)}{\epsilon^2} \right),
    \end{align}
    where $p(\delta) = \Phi^{-1}(1-\delta)$. For instance, for $\delta = 0.001$, $p(\delta) \approx 3$.
    Similarly, if we want each $|\gamma_{ij}^R - \gamma_{ij}| > \epsilon$ with probability at most $\delta$, where $\gamma_{ij}^R$ is the R-sample average estimate of the Gram matrix element $\gamma_{ij}$, then the sample complexity is given by:
    \begin{align}\label{Gsample}
        S_{ij} \gtrapprox O\left(\frac{B_{4L_{ij}} - B_{2L_{ij}}^2}{(L_{ij}!)^4}\sigma^{4L{ij}} \frac{p^2(\delta)}{\epsilon^2} \right).
    \end{align}
    Thus, the sample complexity required is:
    \begin{align}\label{sample_Capp}
        \mathcal{R} = \max \left( \max_i R_i, \max_{i,j} S_{ij} \right).
    \end{align}

    \begin{remark}\label{exp_variance}
    The general summand term in the infinite sum for $\nu_i^2$ (see Lemma 2), say $\nu_i^{2,m,n,p,k} \rightarrow 0$, as $m,n,p,k \rightarrow \infty$ (as well as the terms for the variance $\nu_{ij}^2$). This is necessary for the infinite sum to be convergent and can be shown to be the case using Stirling's formula. However, this does not preclude the variance from becoming very large for some intermediate $N_i$ (respectively $L_{ij}$ for $\nu_{ij}^2$). In particular, the variance is determined by the interplay between the exploration parameter $\sigma$ and the order of the approximation $N_i$/ $L_{ij}$, which is in turn decided by the function that we are trying to approximate. Also, note that we are simply showing the peak variance term in the expressions above and the actual variance will be significantly larger since it is the infinite sum of the individual terms, and thus, the sample complexity expression above is a  rather crude lower bound. Nonetheless, the development above clearly shows that the sample complexity of the solution grows combinatorially-exponentially in the size $\sigma$ of the approximation domain and the order of the approximation required $(N_i, L_{ij})$. \\
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Ill-conditioning:}  
Consider the term $\gamma_{ij}$, and suppose, as above, that the  maximum of the summand is attained when $m=n$ at $K_{ij}$.  
Then,
\begin{align} %\label{conditioning}
\gamma_{ij} &\gtrapprox O\!\left( \frac{B_{2K_{ij}} \, \sigma^{2K_{ij}}}{(K_{ij}!)^2} \right).
\end{align}
However, it is difficult to understand the ill-conditioning issue without an additional assumption. Suppose now that for any $\gamma_{ij}$, the summation is from $m=0:i, n= 0:j$. This implies that the basis functions form progressively higher order approximations, which is typically the case and is  borne out by the empirical evidence in Section \ref{section5}. Then, note that $\gamma_{00} \approx O(1)$, and assuming that the maximum value of $\gamma_{ij}$ over all possible $(i,j)$, when $i=j$, is attained at some $\eta$, and defining $K = K_{\eta\eta}$, an approximate lower bound on the conditioning of the Gram matrix is given as:
\begin{align}\label{conditioning}
    \kappa(\mathcal{G}) \gtrapprox O\!\left( \frac{B_{2K}\sigma^{2K}}{(K!)^2} \right)
\end{align}


If we want to approximate the function $f(.)$ over a suitably large domain, then the exploration parameter $\sigma$ needs to be large as should be the order of approximations $K$ as defined above. Thus, it follows that the Gram matrix $\mathcal{G}$ is highly ill-conditioned, and combined with the variance in the estimates $f_i^R$, the solutions are subject to high variance and consequently unreliable (see Eq. \eqref{ill-cond}).\\

\begin{remark}
The error parameter $\epsilon$ and the confidence level $\delta$ play an identical role here as they do in Probably Approximately Correct (PAC) learning theory \cite{PAC-1,PAC-2}. However, the sample complexity is seen to be combinatorial-exponential in the size of the hypothesis class, in this case, the size of the approximation domain $\sigma$ and the effective order of the approximation $(N_i, L_{ij})$ (see equations \ref{Fsample} and \ref{Gsample} above). Thus, this is not an efficiently learnable problem in the PAC sense since in such a case the dependence has to be polynomial.
\end{remark}




    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Nonlinear Case}\label{nonlinear_theory}
In the following, we show the variance inherent in the gradient estimation and the ill-conditioning of the nonlinear case, the development is almost identical to the linear case.\\
\textbf{Variance:}
The gradient term  in the nonlinear case is given by:
\[
\frac{\partial J}{\partial \theta}
= \mathbb{E} \left[ \Delta(x) \, H(x, \theta) \right],
\]
where
\[
H(x, \theta) =
\begin{bmatrix}
H^{1}(x,\theta) \\
\vdots\\
H^{n}(x,\theta)
\end{bmatrix}
=
\begin{bmatrix}
\frac{\partial h}{\partial \theta_1} \\
\vdots\\
\frac{\partial h}{\partial \theta_p}
\end{bmatrix},
\]
and
\[
\Delta(x) = f(x) - h(x, \theta).
\]

Let
\[
\Delta(x) = \sum_{k=0}^{\infty} \frac{\delta_k}{k!} x^k,
\quad
H^{i}(x) = \sum_{k=0}^{\infty} \frac{h^{i}_k}{k!} x^k.
\]

Then, following the same development as in the linear case,  
the variance in the estimate of the gradient is given by:
\begin{align*}
&\mu_i^2 = \mathrm{Var}(\Delta H^{i}) =\\
\sum_{m,n,r,s}
\frac{\, h^{i}_m \, \delta_n \, h^{i}_r \, \delta_s}
{m! \, n! \, r! \, s!}&\left( B_{m+n+r+s} - B_{m+n} \, B_{r+s} \right) \sigma^{m+n+r+s}.
\end{align*}
In the expression above, given $i$, if the maximum value, when $m=n=p=k$, is attained at $N_i$, the variance is of the order of:
\[
\mu_i^2
\gtrapprox
O\!\left(
\frac{B_{4N_i} - B_{2N_i}^2}{(N_i!)^4} \,
\sigma^{4N_i}
\right).
%\tag{9}
\]
Then, an approximate lower bound on the number of samples required for a given error-confidence level of $(\epsilon, \delta)$ in the gradient estimate with respect to the $i^{th}$ parameter, $\nabla_i^R J$ is given by:
\begin{align}\label{samplecomp}
    R_i \gtrapprox O\left(\frac{B_{4N_i} - B_{2N_i}^2}{(N_i!)^4} \sigma^{4N_i}\frac{p^2(\delta)}{\epsilon^2} \right).
\end{align}
Thus, the sample complexity required: $R = \max_i R_i$, for the error in all the components of the gradient estimate to be within $\epsilon$ with probability at least $1-n\delta$. Hence, it is clear that even in the nonlinear case, the sample complexity of the gradient estimate is exponential-combinatorial in the parameters $(\sigma, N_i)$. \\

\textbf{Ill-conditioning:} In order to show the effect of ill-conditioning in the nonlinear case, consider the following. Let us suppose that the optimal parameter $\theta^*$ is close enough to the current estimate $\Bar{\theta}$ such that a linear expansion about $\Bar{\theta}$, in terms of the perturbation $\delta \theta = \theta - \bar{\theta}$, suffices to approximate $h(x,\theta)$, \textit{i.e.},
\begin{align*}
     &h(x,\theta)\approx h(x,\Bar{\theta})+\underbrace{\begin{bmatrix}
         \frac{\partial h(x,\theta)}{\partial \theta^1} &\cdots &\frac{\partial h(x,\theta)}{\partial \theta^n}
     \end{bmatrix} \Bigg|_{\bar{\theta}} }_{H(x,\bar{\theta})\equiv H} \underbrace{\begin{bmatrix}
         \delta \theta^1 \\ \vdots \\ \delta \theta^n
     \end{bmatrix}}_{\delta {\theta}}. \\
     &\mbox{Define:\;} \epsilon(\theta)= \underbrace{\begin{bmatrix}
         f(x^1)-h(x^1,\bar{\theta})\\ \vdots \\ f(x^R)-h(x^R,\bar{\theta})
     \end{bmatrix}}_{\bar{\Delta}^R} - \underbrace{ \begin{bmatrix}
         H(x^1,\bar{\theta})\\ \vdots \\ H(x^R,\bar{\theta})
     \end{bmatrix} }_{\bar{H}^R} \delta {\theta} 
 \end{align*}

We can rewrite the original cost function in terms of the perturbation variable as: $J(\theta)=\epsilon(\theta)^T \epsilon(\theta)=\epsilon(\delta \theta)^T \epsilon (\delta \theta)\equiv
J(\delta \theta)$. Therefore,
 \begin{equation*}
     J(\delta \theta)=(\Bar{H}^R \delta \theta - \Bar{\Delta}^R)^T (\Bar{H}^R \delta \theta - \Bar{\Delta}^R).
\end{equation*}

Then, the gradient descent algorithm in the vicinity of $\Bar{\theta}$ can be written as:
\begin{align*}
  \delta \theta_t &= \delta \theta_{t-1} - \gamma \frac{\partial J(\delta \theta)}{\partial (\delta \theta)} \\
  &= \delta \theta_{t-1} - \gamma \bar{H}^{R'} (\bar{H}^R \delta\theta-\bar{\Delta}^R),
\end{align*}
which, for small $\gamma$, can be approximated as $\delta \Dot{\theta}=-\bar{H}^{R'}(\bar{H}^R\delta\theta- \bar{\Delta}^R)$. At convergence, $\delta\Dot{\theta}=0$, which implies
\begin{equation}
\label{eq: LSEquiv}
   \delta \theta = (\bar{H}^{R'}\bar{H}^R)^{-1} (\bar{H}^{R'}\Delta^R).
\end{equation}
Note that the above equation has the same least square solution form as the linear case and the empirical Gram matrix in this case is $\mathcal{G}^R = \bar{H}^{R'}\bar{H}^R$, i.e., the matrix $H^R$ containing the derivatives of the nonlinear approximator with respect to the parameters plays the role of the matrix $\Psi^R$ in the linear case, and will have the same ill-conditioning as the linear case.

% Thus, a sequence of gradient-descent steps in the neighborhood of  $\Bar{\theta}$ may be thought of as equivalent to the single linear least squares solution.
\subsection{Multidimensional Case}
In the following, we show how to extend the variance analysis to a multidimensional function. We examine the case of a scalar valued multidimensional function, the extension to the vector valued case is relatively straightforward. Let $\mathbf{x}= (x_1, \cdots x_d) $. Further, let
\begin{align}
f(\mathbf{x}) &= \sum_{\substack{i_1+i_2+\cdots+i_d=n \\ n}}
   \frac{F_{i_1,\dots,i_d}}{i_1! i_2! \cdots i_d!}
   x_1^{i_1} x_2^{i_2} \cdots x_d^{i_d}, \\[1em]
\psi^i(\mathbf{x}) &= \sum_{\substack{i_1+i_2+\cdots+i_d=n \\ n}}
   \frac{\beta^i_{i_1,\dots,i_d}}{i_1! i_2! \cdots i_d!}
   x_1^{i_1} x_2^{i_2} \cdots x_d^{i_d},
\end{align}
denote the multidimensional Taylor series expansions of the function and the basis functions respectively. Then,
\begin{align}
f \psi^i 
&= \sum_{\substack{i_1+i_2+\cdots+i_d = m \\ k_1+\cdots+k_d = n \\
m,n}}
   \frac{F_{i_1,\dots,i_d} \, \beta^i_{k_1,\dots,k_d}}
        {i_1! \cdots i_d! \; k_1! \cdots k_d!}
   x_1^{i_1+k_1} \cdots x_d^{i_d+k_d}.
\end{align}
 To simplify the notation, let $I=\{i_1,\cdots i_d\}$. Further, we will write: $|I| = m$, to denote the sum $\sum_{k=1}^d i_k = m$ and $I!$ to denote the product $\prod_{k=1}^d i_k$ for all possible $I$.\\
 
Next, we assume that $x_1,\dots,x_d$ are sampled independently and each variable is sampled with the same exploration parameter $\sigma$. Then, we obtain the following.
\begin{align}
\mathbb{E}\!\left[ f \psi^i \right] &=f_i(\sigma) \\
&= \sum_{\substack{|I|=m \\ |K| = n \\ m,n}}
   \frac{F_I \,
   \beta^i_K \,}{I!K!}
   B_{i_1+k_1}\sigma^{i_1+k_1} \cdots B_{i_d+k_d}\sigma^{i_d+k_d}.
\end{align}

Next, we can write:
\[
\sigma_i^2=\mathrm{Var}(f \psi^i) 
   = \mathbb{E}\!\left[
      \left(
      \sum_{\substack{|I|=m \\ |K|=n\\ m,n}}
      \tfrac{F_{I}\,\beta^i_{K}}
            {I! \; K!}
      x_1^{i_1+k_1}\cdots x_d^{i_d+k_d} - f^i
      \right)^{\!2}
   \right].
\]

Expanding,
\[
\begin{aligned}
\sigma_i^2
   &= \sum_{\substack{|I|=m,\, |K|=n \\ 
                      |L|=r,\, |P|=s \\ m,n,r,s}}
   \tfrac{F_{I}\,F_{L}\,
          \beta^i_{K}\,\beta^i_{P}}
        {(I!)(K!)(L!)(P!)} \\[0.5em]
   &\quad \times \Bigl[\prod_{r=1}^d B_{i_r+k_r+l_r+p_r} 
       - \prod_{r=1}^d B_{i_r+k_r}\,B_{l_r+p_r}\Bigr]\,
   \sigma^{m+n+r+s}.
\end{aligned}
\]
Suppose now that the maximum value when $m=n=r=s$ is attained at $N_i$, then each term in the sum above is of
$O\!\left( \dfrac{B_{4N_i} - B_{2N_i}^2}{(N_i!)^4} \, \sigma^{4N_i} \right)$. In particular, the value $\dfrac{B_{4N_i} - B_{2N_i}^2}{(N_i!)^4}$ in the $O(.)$ calculation is attained when $i_r=k_r=l_r=p_r=N_i$ for any $r=1,\cdots d$. However, evaluating the other terms, when more than one of the indices is non-zero is intractable. Instead, we substitute the $O(.)$ calculation above and note that this is simply to get a rough idea of the numbers involved.

Since there are $d^{N_i}$ ways in which each of $|I| = N_i$, $|K| = N_i$, $|L| = N_i$, and $|P| = N_i$, there are $d^{4N_i}$ such terms in the sum above.
Hence, it follows that
\[
\sigma_i^2 \gtrapprox O\!\left( \frac{B_{4N_i} - B_{2N_i}^2}{(N_i!)^4} \, (\sigma d)^{4N_i} \right).
\]
An analogous argument shows that $\sigma_{ij}^2 = \mathrm{Var}(\psi^i\psi^j)$ is also of the same order:
\begin{align}
    \sigma_{ij}^2 \gtrapprox O\!\left( \frac{B_{4L_{ij}} - B_{2L_{ij}}^2}{(L_{ij}!)^4} \, (\sigma d)^{4L_{ij}} \right),
\end{align}
where $L_{ij}$ is defined in an identical manner to the scalar case. The sample complexity is then given by equations \ref{Fsample}, \ref{Gsample} and \ref{sample_Capp}.

Finally, the conditioning of the problem is given by: 
\[
\kappa(\mathcal{G}) \gtrapprox O\!\left( \frac{B_{2K}}{(K!)^2} \, (\sigma d)^{2K} \right),
\]
with an analogous definition of $K$ as in the scalar case.
 We see that the dimension affects the variance and conditioning of the problem by effectively amplifying the exploration parameter $d$ times. \\
 \begin{remark}
 A note is due regarding the independent sampling in the different dimensions. It is always possible to linearly transform any set of correlated random variables such that they are uncorrelated and have the same variance, and thus, the variance expression above will still hold albeit the variables are uncorrelated, in general, and not necessarily independent. The resulting variables become independent if the sampling is Gaussian.\\
 \end{remark}
 
 \begin{remark}
     The extension of the multidimensional variance and ill-conditioning analysis to the nonlinear case can be done in a relatively straightforward fashion using the analysis in the scalar case and is left out for brevity.
 \end{remark}
%\section{Data Driven Solutions}
%\label{sec3}


%\textcolor{red}{Make all equations, except the important ones, inline.}

%\subsection{Heuristic Idea} In the following, we shall show that approximating $f(\cdot)$ globally, equivalently, to a high polynomial order, is identical to finding the generalized higher order moments of the state $x$, under the sampling density $p(\cdot)$. In particular, the elements of the Gram matrix $\mathcal{G}_{ij}$ are moments of the underlying state: $\mathcal{G}_{11}$ corresponds to the first moment while $\mathcal{G}_{nn}$ corresponds to the $2n^{th}$ moment, and thereby, $\mathcal{G}_{11} \ll \mathcal{G}_{nn}$, leading to severe ill-conditioning of the Gram matrix. Further, $\langle f,\psi_n \rangle$ is the $2n^{th}$ order moment of the state $x$, and thus, its variance is the $4n^{th}$ order moment. Noting that moments grow combinatorially-exponentially in the order of the approximation, for instance, for Gaussian random variables, they grow as $(2n)!!\sigma^{2n}$, where $\sigma^2$ is the variance of the underlying sampling density, this implies that the number of samples required to get reliable estimates of the projections grows in a combinatorial-exponential fashion. Thus, the right hand side of the Normal equation $\mathcal{G}C = F$ has high variance while the Gram matrix is ill-conditioned and has high variance, and thus, the solution is bound to be subject to large errors. Moreover, owing to the same reason, there is a lack of convergence of such models, i.e, different datasets lead to different models when approximating to a high order. Further, it is not clear what the sampling distribution ought to be. Thus, in order to combat these issues with estimating nonlinear ``global" models, to solve nonlinear optimal control problems, it is sufficient %necessary and sufficient 
%that we identify local LTV systems by sampling ``locally" around our current estimate of the optimal control trajectory and iterating till convergence as in the ILQR approach.

%\subsection{Linear Case: Variance and Ill-Conditioning}


%\subsection{Ill-Conditioning and Variance of the Linear Solution}
%\label{sec:Conditioning_LLS}
% \textcolor{red}{Make sure all the $g_{kl}$/ $g$ variables are changed to $\mathcal{G}_{kl}$/ $\mathcal{G}$.}
%Thus, we shall show how this variance scales for some common choices of basis functions. In essence, we shall show that the data-based solution suffers from very high variance as well as severe ill-conditioning. Note that $(\frac{1}{R}\underline{\Psi}^{R'}F^R)_i= f_i^R$ and $(\frac{1}{R}\underline{\Psi}^{R'}\underline{\Psi}^{R})_{ij}=G_{ij}^R$, where $i,j=1,2...N$.
% \begin{bmatrix}
%     f_1^R\\ \vdots \\ f_N^R
% \end{bmatrix}$ and $\frac{1}{R}\underline{\Psi}^{R'}\underline{\Psi}^{R}= \begin{bmatrix}
%     \mathcal{G}_{11}^R &\hdots &\mathcal{G}_{1N}^R\\
%     \vdots & &\vdots\\
%     \mathcal{G}_{N1}^R &\hdots &\mathcal{G}_{NN}^R
% \end{bmatrix}$.

%\subsection{Global Approximation/Expansion to a High-Order}
%Let us suppose we want to expand the function $f(x)$ in some region $D\subset\mathbb{R}$. As the size of the domain $D$ increases, we need to correspondingly expand the function $f(\cdot)$ to a higher-order (polynomial) in order to assure accuracy, \textit{i.e.}, %$f(x)\approx a_0 + a_1 x+...+a_N x^N \text{, } \forall x\in D$.
%\begin{equation*}
 %   f(x)\approx a_0 + a_1 x+...+a_N x^N \text{, } \forall x\in D.
%\end{equation*}

%However, $f(\cdot)$ may be expanded in some other basis as well, say $\{\psi_1(x)...\psi_N(x)\}$. Nonetheless, \begin{equation*}
 %   Span\{\psi_1...\psi_N\}=Span\{1,x,...,x^N\},
%\end{equation*}%$Span\{\psi_1...\psi_N\}=Span\{1,x,...,x^N\}$, 
%and any 
%\begin{equation*}
 %   \psi_k(x)\approx \alpha_0^k +\alpha_1^k x+...+\alpha_N^k x^N,
%\end{equation*} given that the support of the basis $\psi_k(\cdot)$ is over the entire domain $D$, \textit{i.e.}, they are not ``localized" functions/ ``local approximations".

%Thus, $f(x)\psi_k(x)\sim O(x^{2N})$ and $\psi_k(x)\psi_l(x)\sim O(x^{2N})$, \textit{i.e.}, these products are polynomials of order $2N$. Thus, the corresponding variances $Var[f(x)\psi_k(x)]$ and $Var[\psi_k(x)\psi_l(x)]$ are determined by the $(4N)^{th}$ order moment of $x$.

%\subsubsection{Monomial Basis}
%Suppose that our basis set $\Psi=\{1,x,...,x^N\}$ be the set of monomials, \textit{i.e.}, we approximate $f(\cdot)$ by an $n^{th}$ order polynomial.
%Let us assume that our sampling distribution $p(x)\sim N(0,\sigma_x^2)$, \textit{i.e.}, the sampling distribution is normal with variance $\sigma^2$. Now, $f(x)\psi_k(x)\sim O(x^{k+N})$. %Therefore, 
%\begin{align*}
 %$   Var[f(x)\psi_k(x)] = \underbrace{O((2(k+n)-1)!!\sigma^{2(k+n)})}_{\text{if $k+n$ is odd}},%\\
  %  \text{or}$\\
    %$\underbrace{O([(2(k+n)-1)!!-(k+n-1)!!^2]\sigma^{2(k+n)})}_{\text{if $k+n$ is even}},\, 
%$%\end{align*}
 %where $k!! = 1\cdot3\cdot 5 ... \cdot k$. 
%Thus, we need $R\sim O([(4N-1)!!-(2N-1)!!^2 \sigma_x^{4N}])$ samples for $\langle f,\psi_N \rangle$ to converge (the number within the $O(.)$ is the variance of $x^{2N}$). This implies that, in order to approximate $f(\cdot)$, to a high-order ``N", the samples required are combinatorial-exponential in the order.

%\subsubsection{Orthonormal Basis}
%{Suppose now that our basis set is defined as the set of normalized Hermite polynomials for a Gaussian sampling distribution, or the Legendre polynomials with a uniform sampling distribution. The corresponding sampling complexity for the Hermite basis is %$ R\sim O\Bigg(\frac{[(4N-1)!!-(2N-1)!!^2]}{(N!)^2} \sigma_x^{2N} \Bigg)$
%\begin{equation*}
%    R\sim O\Bigg(\frac{[(4N-1)!!-(2N-1)!!^2]}{(N!)^2} \sigma_x^{2N} \Bigg),
%\end{equation*} while the Legendre basis results in a sample complexity of %$R\sim O\Bigg(\frac{(2N)!^2 4N^2}{(N!)^4 (2N+1)^2 (4N+1)} \sigma_x^{2N} \Bigg)$
%\begin{equation*}
  %  R\sim O\Bigg(\frac{(2N)!^2 4N^2}{(N!)^4 (2N+1)^2 (4N+1)} \sigma_x^{2N} \Bigg).
%\end{equation*} Thus, despite a significantly reduced sampling complexity, the samples required are nonetheless combinatorial-exponential.}

% \subsubsection{Hermite Basis (Orthonormal)}
% Suppose now that our basis set $\Psi=\{h_0(x),h_1(x),...,h_n(x)\}$ be the set of normalized Hermite polynomials. It is well-known that the Hermite polynomials form the orthonormal basis for Gaussian sampling distributions. Assuming the same normal sampling distribution $p(\cdot)$, we have the corresponding sample complexity 
% $ R\sim O\Bigg(\frac{[(4N-1)!!-(2N-1)!!^2]}{(N!)^2} \sigma_x^{2N} \Bigg)$
% % \begin{equation*}
% %     R\sim O\Bigg(\frac{[(4N-1)!!-(2N-1)!!^2]}{(N!)^2} \sigma_x^{2N} \Bigg)
% % \end{equation*}
% for approximating $f(\cdot)$ as a linear combination of the first $N$ normalized Hermite polynomials. Thus, using an orthonormal basis results in a significantly reduced sampling complexity, but the samples required are still combinatorial-exponential.

% \subsubsection{Legendre Basis (Orthonormal)}
% Similar to the Hermite polynomials, the Legendre polynomials form the orthonormal basis for a uniform sampling distribution. Suppose that our basis set $\Psi=\{L_0(x),L_1(x),...,L_n(x)\}$ is now the set of Legendre polynomials. Let us also assume that the sampling distribution is now uniform, i.e. $p(\cdot)=\frac{1}{\sigma_x}$. Then, the corresponding sample complexity is $R\sim O\Bigg(\frac{(2N)!^2 4N^2}{(N!)^4 (2N+1)^2 (4N+1)} \sigma_x^{2N} \Bigg)$
% % \begin{equation*}
% %     R\sim O\Bigg(\frac{(2N)!^2 4N^2}{(N!)^4 (2N+1)^2 (4N+1)} \sigma_x^{2N} \Bigg)
% % \end{equation*}
% if expanding $f(\cdot)$ to order $N$ in the Legendre polynomials.
%\subsubsection{Ill conditioning}
%Let us now take a look at the conditioning of the Gram matrix. Upon using a suitable basis set $\Psi$, the diagonal elements of the Gram matrix $G = \Psi' \Psi$ are $O(E[x^0]),O(E[x^2]), ...,O(E[x^{2N}]$.
% \begin{bmatrix}
%     O(E[x^0]) &\hdots &0\\
%      &\ddots &\\
%     0 &\hdots &O(E[x^{2N}])
% \end{bmatrix}$
%The condition number is then determined by $\frac{G_{NN}}{G_{11}}=O(E[x^{2N}])$. For instance, given that the sampling distribution is zero-mean Gaussian, the conditioning
%of $O((2N)!!\sigma_x^{2N})$.

%\subsection{The Nonlinear Case}
%\label{sec:Conditioning_Nonlinear}


%Note that the typical gradient-descent algorithm is
%\begin{equation}
%\label{eq: Gradient-Descent}
 %   \theta_{t+1}=\theta_t- \gamma \frac{\partial J}{\partial \theta}\Bigg|_{\theta_t} .
%\end{equation}
%5Assuming step-size $\gamma$ to be small, the trajectory of the algorithm can be approximated by the ODE $\Dot{\theta}=-\frac{\partial J}{\partial \theta}$, where, at convergence, $\Dot{\theta}= 0$, and hence, the algorithm converges to a stationary point of the cost function.
%\subsubsection{Gradient Descent as Recursive Least-Squares}
%\textcolor{red}{You can simply state Eq. 11 and cut the preceding development.}
% We can consider the gradient-descent algorithm as a succession of recursive Linear Least-Squares steps. In order to see this, let $\{(x^1,f(x^1)),...,(x^R,f(x^R))\}$ be the given data-set, and let the current parameter value of the approximation architecture $h(x,\theta)$ be $\Bar{\theta}$. Then, define the approximation error $ \epsilon(\theta)=\begin{bmatrix}
%         f(x^1)\\ \vdots \\ f(x^R)
%     \end{bmatrix} - \begin{bmatrix}
%         h(x^1,\theta)\\ \vdots \\ h(x^R,\theta)
%     \end{bmatrix}$.
% % \begin{equation*}
% %     \epsilon(\theta)=\begin{bmatrix}
% %         f(x^1)\\ \vdots \\ f(x^R)
% %     \end{bmatrix} - \begin{bmatrix}
% %         h(x^1,\theta)\\ \vdots \\ h(x^R,\theta)
% %     \end{bmatrix} .
% % \end{equation*}

% Now, let us suppose that the parameter $\theta$ remains close enough to $\Bar{\theta}$ such that a linear expansion about $\Bar{\theta}$, in terms of the perturbation $\delta \theta = \theta - \bar{\theta}$, suffices to approximate $h(x,\theta)$, \textit{i.e.},
% \begin{align*}
%     &h(x,\theta)=h(x,\Bar{\theta})+\underbrace{\begin{bmatrix}
%         \frac{\partial h(x,\theta)}{\partial \theta^1} &\hdots &\frac{\partial h(x,\theta)}{\partial \theta^n}
%     \end{bmatrix} \Bigg|_{\Bar{\theta}} }_{H(x,\Bar{\theta})\equiv H} \underbrace{\begin{bmatrix}
%         \delta \theta^1 \\ \vdots \\ \delta \theta^n
%     \end{bmatrix}}_{\delta {\theta}} \\
%     &\implies \epsilon(\theta)= \underbrace{\begin{bmatrix}
%         f(x^1)-h(x^1,\Bar{\theta})\\ \vdots \\ f(x^R)-h(x^R,\Bar{\theta})
%     \end{bmatrix}}_{\Bar{\Delta}^R} - \underbrace{ \begin{bmatrix}
%         H(x^1,\Bar{\theta})\\ \vdots \\ H(x^R,\Bar{\theta})
%     \end{bmatrix} }_{\Bar{H}^R} \delta {\theta} \\
%     &\implies \epsilon(\theta)=\epsilon(\delta {\theta})=\Bar{\Delta}^R - \Bar{H}^R \delta {\theta}.
% \end{align*}

% Now, we can write the cost function as $J(\theta)=\epsilon(\theta)^T \epsilon(\theta)=\epsilon(\delta \theta)^T \epsilon (\delta \theta)\equiv
% J(\delta \theta)$. Therefore, $J(\delta \theta)=(\Bar{H}^R \delta \theta - \Bar{\Delta}^R)^T (\Bar{H}^R \delta \theta - \Bar{\Delta}^R)$.
% % \begin{equation*}
% %     J(\delta \theta)=(\Bar{H}^R \delta \theta - \Bar{\Delta}^R)^T (\Bar{H}^R \delta \theta - \Bar{\Delta}^R).
% % \end{equation*}

% Then, the gradient descent algorithm in the vicinity of $\Bar{\theta}$ can be construed as $\delta \theta_t = \delta \theta_{t-1} - \gamma \frac{\partial J(\delta \theta)}{\partial (\delta \theta)} = \delta \theta_{t-1} - \gamma \Bar{H}^{R'} (\Bar{H}^R \delta\theta-\Bar{\Delta}^R)$,
% % \begin{align*}
% %     \delta \theta_t &= \delta \theta_{t-1} - \gamma \frac{\partial J(\delta \theta)}{\partial (\delta \theta)} \\
% %     &= \delta \theta_{t-1} - \gamma \Bar{H}^{R'} (\Bar{H}^R \delta\theta-\Bar{\Delta}^R),
% % \end{align*}
% which, for some small $\gamma$, can be approximated as $\delta \Dot{\theta}=-\Bar{H}^{R'}(\Bar{H}^R\delta\theta- \Bar{\Delta}^R)$. At equilibrium, $\delta\Dot{\theta}=0$, which implies
% \begin{equation}
% \label{eq: LSEquiv}
%     \delta \theta = (\Bar{H}^{R'}\Bar{H}^R)^{-1} (\Bar{H}^{R'}\Delta^R).
% \end{equation}

% Thus, a sequence of gradient-descent steps in the neighborhood of  $\Bar{\theta}$ may be thought of as equivalent to the single linear least squares solution.
% Therefore, the gradient descent algorithm, owing to Eq.~\ref{eq: LSEquiv} may be treated as a sequence of linear least-squares solutions with a suitable learning rate:
%{The gradient-descent algorithm can be considered as a succession of recursive Linear Least-Squares solutions with a suitable learning rate:}
%\begin{equation}
%\label{eq:LSSol_nonlinear}
 %   \theta_{t+1}=\theta_t+ \alpha(\Bar{H}_{t}^{R'}\Bar{H}_{t}^R)^{-1} (\Bar{H}_{t}^{R'}\Delta_{t}^R)
%\end{equation}
%where $(H_{t}^R)_{ij}=\frac{\partial h(x^i,\theta)}{\partial \theta^j}\Bigg|_{\theta_{t}}$ and $(\Delta_{t}^R)_i=f(x^i)-h(x^i,\theta_{t})$ for $i=1,2...R$, and $j=1,2...n$. \\
% where $H_{t}^R=\begin{bmatrix}
% \frac{\partial h(x^1,\theta)}{\partial \theta^1} & \hdots & \frac{\partial h(x^1,\theta)}{\partial \theta^n} \\
% \vdots & &\vdots \\
% \frac{\partial h(x^R,\theta)}{\partial \theta^1} &\hdots &\frac{\partial h(x^R,\theta)}{\partial \theta^n}
% \end{bmatrix} \Bigg|_{\theta_{t}}$ and $\Delta_{t}^R=\begin{bmatrix}
%     f(x^1)-h(x^1,\theta_{t})\\ \vdots \\ f(x^R)-h(x^R,\theta_{t})
% \end{bmatrix}$. \\

%Thus, Eq.~\ref{eq:LSSol_nonlinear} amounts to approximating $\Delta_{t}^R$ in the basis $H_{t}^R$ for every step $t$.

%\paragraph{Variance} Note that, as before, $\Delta_t$ will be a high order function when trying to approximate $f(.)$ in a global fashion. In particular, note that the error function is $\Delta_t(x) = (f(x)-h(x,\theta_t))$
% \begin{equation*}
%     \Delta_t(x) = (f(x)-h(x,\theta_t))
% \end{equation*}
%and we approximate $\Delta_t$ in the linear subspace spanned by $\{H_t^1(x)...H_t^n(x)\}$, where $H_T^i(x)=\frac{\partial h}{\partial \theta^i}\Bigg|_{\theta_t}$. When approximating in a global fashion (to a high order), both $\Delta_t$ and $H_t^p$ will be high order. Also, we further note that $\frac{1}{R}H_t^{R'}\Delta_t^R = \frac{1}{R}\sum_{k=1}^R H_t^i(x^k)\Delta_t(x^k)\approx \langle H_t^i,\Delta_t \rangle=\int H_t^i(x)\Delta_t(x)p(x)dx$.
% \begin{eqnarray*}
%     \frac{1}{R}H_t^{R'}\Delta_t^R = \frac{1}{R}\sum_{k=1}^R H_t^i(x^k)\Delta_t(x^k)\approx<H_t^i,\Delta_t>\\
%     =\int H_t^i(x)\Delta_t(x)p(x)dx.
% \end{eqnarray*}

%However, if $\Delta_t, H_t^p$ are $O(x^N)$ and $p(\cdot)$ is Gaussian, the variance is $O([(4N-1)!!-(2N-1)!!^2]\sigma^{4N})$ as in the linear case.

%\paragraph{Ill-conditioning}
%In general, the basis functions $H_t^i$ can be of very different orders, and the Gram-matrix $G_t$ thus formed will be highly ill-conditioned as well as subject to high variance as in the linear approximation case. 
%Thus, as before, the update $\delta \theta_t$, at all times $t$, and thus, the final answer will suffer from large variance.

% \vspace{-0.15cm}
\subsection{Recursive Linear Time-Varying Models}
Thus far, we have seen that if we want a high-order/global approximation of a function $f(x)$, by sampling from a given distribution $p(\cdot)$, we are bound to suffer from high variance and ill-conditioning. %However, it is not clear what this distribution ought to be, the data generation issue \cite{schoukens2019nonlinear}. Moreover, the least squares solution is also, in general, dependent on the sampling distribution. 
In the following, we show that if we estimate local LTV models, then the sampling distribution is immaterial, while we are assured of accurate model estimates. Nonetheless, in spite of its local nature, when applied recursively, this approach can be used to accurately solve the motivating optimal control problem.

Let us recall the optimal control problem (Sec.~\ref{probform}) that was the original motivation of our work. Again, assume that $x_0$ is given to us, as is an initial guess for the optimal control (say $\{u_t^0\}$). Suppose that we perturb the system as $x_0+\delta x_0$, and $u_t+\delta u_t$, where $\delta x_0 \sim p_0^x(\cdot)$ and $\delta u_t \sim p_t^u(\cdot)$, and the sampling distributions are small enough ($\sigma$) such that the system is arbitrarily well approximated as linear, \textit{i.e.}, $\delta x_{t+1}\approx A_{t}\delta x_{t}+B_{t}\delta u_{t}$. Note that this is always feasible owing to Proposition \ref{ME_acc}. 
% \begin{equation}
%     \delta x_{t+1}\approx A_{t}\delta x_{t}+B_{t}\delta u_{t}.
% \end{equation}
Then, one may perform roll-outs to get sample trajectories: $ \delta x_{t+1}\approx A_{t}\delta x_{t}^i+B_{t}\delta u_{t}^i\implies \underbrace{\begin{bmatrix}
        \delta x_{t+1}^1 \\ \vdots \\ \delta x_{t+1}^R 
    \end{bmatrix}}_{\delta x_{t+1}^R} = \underbrace{\begin{bmatrix}
        \delta x_{t}^1  &\delta u_t^1 \\ \vdots &\vdots \\ \delta x_{t}^R &\delta u_t^R
    \end{bmatrix}}_{\delta X_{t}^R} \begin{bmatrix}
        A_t \\ B_t
    \end{bmatrix} 
    \implies \begin{bmatrix}
        \Hat{A}_t \\ \Hat{B}_t
    \end{bmatrix} = (\delta X_t^{R'}\delta X_t^R)^{-1} (\delta X_t^{R'}\delta x_{t+1}^R)$. 
% \begin{align*}
% \label{eq:LTV-LS}
%     & \delta x_{t+1}\approx A_{t}\delta x_{t}^i+B_{t}\delta u_{t}^i \\
%     \implies & \underbrace{\begin{bmatrix}
%         \delta x_{t+1}^1 \\ \vdots \\ \delta x_{t+1}^R 
%     \end{bmatrix}}_{\delta x_{t+1}^R} = \underbrace{\begin{bmatrix}
%         \delta x_{t}^1  &\delta u_t^1 \\ \vdots &\vdots \\ \delta x_{t}^R &\delta u_t^R
%     \end{bmatrix}}_{\delta X_{t}^R} \begin{bmatrix}
%         A_t \\ B_t
%     \end{bmatrix} \\
%     \implies &\begin{bmatrix}
%         \Hat{A}_t \\ \Hat{B}_t
%     \end{bmatrix} = (\delta X_t^{R'}\delta X_t^R)^{-1} (\delta X_t^{R'}\delta x_{t+1}^R)
% \end{align*}
The empirical Gram matrix $(\delta X_t^{R'}\delta X_t^R)$ is well-conditioned as $N=1$ and $\sigma$ is small (see \eqref{conditioning}), and the variance in $(\delta X_t^{R'}\delta x_{t+1}^R)$ is low for the same reason (see \eqref{varianceF} and \eqref{varianceG}). Thus, we can estimate the LTV system $(A_t^0,B_t^0)$ around the trajectory generated from $(x_0,\{u_t^0\})$ in an accurate fashion.
%\textcolor{red}{I think we should be able to show that the answer is invariant to the sampling distribution if linearity holds as above.}
However, this only gives us a local description of the system around the initial trajectory $(x_t^0, u_t^0)$. Thus, one may question the practicality of such a local approximation. 
However, in order to find an improved control sequence (see the ILQR algorithm in the appendix), $u_t^1 = u_t^0+\delta u_t^0$, along with a perturbation feedback $K_t^1 \delta x_t$, we need only the local description $(A_t^0, B_t^0)$ around the initial trajectory. Thus, this estimate can be used to find a new control and perturbation feedback sequence $\{u_t^1, K_t^1\}$ which, in turn, defines a new trajectory $\{x_t^1\}$ around which one can find the LTV approximations $\{A_t^1, B_t^1\}$, and so on in an iterative fashion till convergence (Fig.~\ref{fig:optcontrol} (a)-(b)). Thus, this shows that local LTV models suffice for optimal control, and moreover are necessary owing to the ill-conditioning and variance in estimating ``global or higher order models" in a data-based fashion.\\
The `local' model-based RL approach outlined above is called the Decoupled Data-based Control (D2C) and more details regarding this approach can be found in the reference \cite{D2C_ASME}.

% \begin{figure}[!htb]
% % \vspace{-0.3}
% % \begin{multicols}{2}

%       \subfloat[Pendulum Angle]{\includegraphics[width=0.5\linewidth]{figure/Pendulum_neighbour1_2.png}}    
%       \subfloat[Angular Velocity]{\includegraphics[width=0.5\linewidth]{figure/Pendulum_neighbour2_2.png}}
      
% % \end{multicols}

% \caption{{The iterative optimization of the trajectory through algorithms like ILQR results in significantly different trajectories during optimization, and thus, the corresponding LTV models are significantly different as the optimization proceeds.}}
% \vspace{-0.4cm}
% \label{fig:TrajVariation}
% \end{figure}

==> improvements.tex <==
\section{Improvement in system identification: Number of Rollouts}\label{sec_alg}

Intro to using LLS-CD to find $A_t$ and $B_t$ in the full vs reduced order model.

The system identification problem thus reduces from an $O(n_x+n_u)$ problem to $O(n_\alpha + n_u)$ problem, where $n_\alpha<< n_x$.



==> test.tex <==
% After getting the local LTV parameters about the system, the ILQR algorithm computes a local optimal control by solving the following discrete time Riccati Equation, which is given by
% \begin{align}
%     \delta u_t
%     %&=R^{-1}f_{u_t}'(-v_{t+1}-V_{t+1}\delta x_{t+1})-\bar{u}_t \nonumber \\
%     &=R^{-1}B_t^T(-v_{t+1}-V_{t+1}(A_t\delta x_t + B_t\delta u_t))-\bar{u}_t, \nonumber \\
%     &=-(R+B^T_t V_{t+1}B_t)^{-1}(R\bar{u}_t+B_t^T v_{t+1}\nonumber \\
%     &+B_t^T V_{t+1}A_t\delta x_t),
% \end{align}
% which can be written in the linear feedback form $\delta u_t =-k_t-K_t\delta x_t$, where $k_t=(R+B_t^T V_{t+1}B_t)^{-1}(R\bar{u}_t+B_t^T v_{t+1})$ and $K_t=(R+B_t^T V_{t+1}B_t)^{-1}B^T_t V_{t+1}A_t$, and
% \begin{subequations}
% \begin{align}
%     v_t &= l_{t,x}+A_t^T v_{t+1}-A_t^T V_{t+1}B_t(R+B_t^T V_{t+1}B_t)^{-1}\nonumber \\
%     &\cdot(B_t^T v_{t+1}+R\bar{u}_t) \label{eq:vt}\\
%     V_t &= l_{t,xx}+A_t^T (V_{t+1}^{-1}+B_t R^{-1}B_t^T)^{-1}A_t\nonumber \\
%     &=l_{t,xx}+A_t^T V_{t+1}A_t-A_t^T V_{t+1}B_t(R+B_t^T V_{t+1}B_t)^{-1} \label{eq:Vt} \nonumber \\
%     &\cdot B_t^T V_{t+1}A_t.
% \end{align}
% \end{subequations}
% with the terminal conditions $v_T(x_T)=\frac{\partial c_T}{\partial x}|_{x_T}=\frac{\partial l}{\partial x}|_{x_T}$ and $V_T(x_T)=\nabla ^2_{xx}c_T|_{x_T}$. To compute $v_t$ and $V_t$, we need their corresponding values in the future, \textit{i.e.} $v_{t+1}$ and $V_{t+1}$. From Eqs. \ref{eq:vt} and \ref{eq:Vt} we see that, given the terminal conditions and the local LTV model parameters $(A_t, B_t)$, we can do a backward-in-time sweep to compute all values of $v_t$ and $V_t$, and thus, the corresponding optimal control for that trajectory.
